When Cyber-Physical Systems Meet AI: A Benchmark, an Evaluation, and a Way Forward

Cyber-physical systems (CPS) have been broadly deployed in safety-critical domains, such as automotive systems, avionics, medical devices, etc. In recent years, Artificial Intelligence (AI) has been increasingly adopted to control CPS. Despite the popularity of AI-enabled CPS, few benchmarks are publicly available. There is also a lack of deep understanding on the performance and reliability of AI-enabled CPS across different industrial domains. To bridge this gap, we initiate to create a public benchmark of industry-level CPS in seven domains and build AI controllers for them via state-of-the-art deep reinforcement learning (DRL) methods. Based on that, we further perform a systematic evaluation of these AI-enabled systems with their traditional counterparts to identify the current challenges and explore future opportunities. Our key findings include (1) AI controllers do not always outperform traditional controllers, (2) existing CPS testing techniques (falsification, specifically) fall short of analyzing AI-enabled CPS, and (3) building a hybrid system that strategically combines and switches between AI controllers and traditional controllers can achieve better performance across different domains. Our results highlight the need for new testing techniques for AI-enabled CPS and the need for more investigations into hybrid CPS systems to achieve optimal performance and reliability.

==> sections-old/approach.tex <==
\section{Methodology}\label{sec:methodology}
\begin{figure*}
    \centering
    % \includegraphics[width=1\linewidth]{pics/pathoverview.pdf}
    \includegraphics[width=1\linewidth]{pics/pathoverview_v2_tight_fx.pdf}
    \caption{Overview of this work.}
    \label{fig:overview}
\end{figure*}

\subsection{Overview}
To design coverage criteria that are related to the decision logic of DNN, it is necessary to understand the decision-making of the black-box DNN (we say DNN is black-box since it is usually uninterpretable). Fortunately, some recent progress has been made on the interpretation of the machine learning models~\cite{bach2015pixel,fong2017interpretable,wang2018interpret}, which can be used for the interpretable coverage criterion.

In this work, we applied the \textit{Layer-Wise Relevance Propagation} (LRP)~\cite{bach2015pixel} to reveal the internal decision of an input.
LRP is an effective approach that interprets the classification decisions by the decomposition of nonlinear classifiers (\eg, DNNs) such that the key features in the input (\eg, pixels in the images) could be identified.
%which are the main contributions for the decision, could be identified.
In particular, given an input, LRP calculates the \textit{relevance} of neurons in each layer starting from the last layer to the input layer in terms of the prediction result. The relevance represents the effect of neurons in the decision. Based on the relevance, we define the \textit{Critical Decision Path} (CDP) that is a set of critical neurons (\ie, with larger relevance from each layer) for the decision. Consider the left figure in Fig.~\ref{fig:motivating}(b) as an example, the yellow path and the red path represent different decision logic for the prediction of dogs and cats, respectively. Our evaluation results show that similar inputs (\eg, dogs) tend to share a similar CDP (\ie, their decision logic is similar) while different inputs (\eg, dogs and cats) have different CDPs.

Inspired by the path coverage in software testing, we propose the Neuron Path Coverage (NPC). For example, in the control flow graph of Fig.~\ref{fig:motivating}(a), it returns the maximum value of the inputs $x$ and $y$. The two paths show the clear logic of the program: the left path represents that $x$ is the larger one while the right path represents that $y$ is the larger one. Similarly, the extracted CDPs are used to show the logic of the DNN. For ease of understanding, we show a dummy graph in the right figure of Fig.~\ref{fig:motivating}(b), if the input executes the yellow path, it is classified as the cat, otherwise, a dog.
%Intuitively, in DL testing, the high neuron path coverage indicates that more different CDPs are covered, \ie, more decision logic is explored by the test cases.

Fig.~\ref{fig:overview} shows the more detailed workflow of our work. The decision logic of the DNN is determined by the training data, given the target DNN, we first individually extract the CDP for each training data (Section~\ref{sec:pathextract}). 
The extracted CDPs represent the decision logic that is learned from the training data. Given an input, we measure the coverage by calculating the distance between the CDP of a given input and CDPs of training data (\ie, the difference of the decision logic). However, calculating the distance with all training samples is computationally expensive. To improve the efficiency, we perform the intra-class path clustering and abstraction on the CDPs of training samples (Section~\ref{sec:pathabstract}). 
Specifically, the assumption is that the samples with similar decision logic may have similar CDP. Thus, for the inputs predicted as the same class, we group their CDPs into $k$ clusters. It means that inputs with similar decision logic are clustered into one group. For example, the similar cats are clustered together (\eg, the yellow cats and brown cats in Fig.~\ref{fig:overview}).
For each cluster, we further propose the path abstraction that merges CDPs of inputs (in the cluster) into an abstract CDP. The abstract CDP represents the decision logic for all inputs in this cluster. Finally, the number of paths is greatly reduced. 
Based on the abstract CDPs, we propose the distance-based coverage criteria (Section~\ref{sec:criteria}), which measure to what extent new decision logic is covered by the given test suite. Specifically, we first identify the abstract CDP of the given input and then propose two coverage criteria. From the control-flow perspective, we calculate the \textit{similarity} between the new CDP and the abstract CDP of the corresponding cluster. From the data-flow perspective, we take the activation value of neurons in the abstract CDP into consideration and calculate the \textit{distance} (along the abstract CDP) between the input and training samples in the cluster. The similarity and distance reveal how different the decision behavior of the new input is.
Similar to~\cite{test:surprise}, we divided the similarity/distance to $m$ buckets and calculate how many buckets are covered by a given test suite. \revise{To adopt the coverage criteria in testing DNNs, we need to select the optimal hyperparameters for the CDP extraction and abstraction. We propose a method to select the parameters by evaluating the accuracy of the CDPs on affecting the decision. }
% To be more fine-grained, we consider the output values along the CDP and 

% by calculating the distance between the CDP of the given nearest  the CDP of the new test input and CDPs of the training samples. 

 
%distance between the  Given a new input, we calculate the distance between its CDP and all abstract CDPs. 




%To calculate the NPC, one challenge is that the number of the CDPs may be infinite, which is similar with the programs (\eg, the loop may cause the program paths infinite). Following the strategy~\cite{pathcov,test:surprise} that bound the infinite coverage by a parameter, we propose the distance-based NPC. Specifically, the NPC of a test suite is calculated by measuring the distance between the CDP of the test case and CDPs of the training samples. Then the distance is discretized to the finite number of buckets for calculating the coverage. 


\subsection{Path Extraction}\label{sec:pathextract}
In this section, we will introduce how to extract the critical decision path for a given input.

% \begin{definition}[Deep Neural Network]\label{def:dnn}
% A Deep Neural Network (DNN) $f$
% consists of multiple layers $\left\langle l_1,\ldots,l_n\right\rangle$, where $l_1$ is the input layer, $l_n$ is the output layer, and $l_2,\ldots,l_{n-1}$ are hidden layers. The inputs of each layer are from outputs of previous layers.
% \end{definition}

% In this work, we mainly focus on the classifier $f:X \rightarrow Y $, where $X$ is a set of inputs and $Y$ is a set of classes.  Given an input $x\in X$, $f(x)=\argmax_{y}O_n(y)$, where $O_n$ is a $|Y|$-dimensional vector, which is the output of the output layer $l_n$. The input is classified as the class $y$, and we use $g_f(x)=O_n(y)$ to represent the output value (\eg, the logits) for the class $y$.
% %The output $y\in Y$ is the final prediction of the classifier.
% Due to the complex non-linear calculation in the DNN, it is hard to understand the decision.

% Layer-Wise Relevance Propagation (LRP)~\cite{bach2015pixel} is an effective way to interpret the decision by calculating the key features in the input. Given an $d$-dimensional input $x$ and the classifier $f$, LRP calculates the relevance of each dimension in the input: $g_f(x)\approx \sum_{i=1}^{d} R_i^{l_1}$, where $g_f(x)$ is the output value of the prediction and $R_i^{l_1}$ represents the relevance of the dimension $i$ in the input layer $l_1$ (\eg, the pixel in an image). The qualitative interpretation is that $ R_i^{l_1}<0$ contributes evidence against the presence of the class which is to be classified while $ R_i^{l_1}>0$ contributes evidence for its presence~\cite{bach2015pixel}. 
% The relevance is calculated by a layer-by-layer backward propagation (from the output layer $l_n$ to the input layer $l_1$) such that:
% $$g_f(x)=R_y^{l_n} = \sum_{i\in{l_{n-1}}} R_i^{l_{n-1}} = \ldots = \sum_{i\in{l_1}} R_i^{l_1}$$
% where $R_i^{l}$ represents the relevance of the neuron $i$ at the layer $l$. The relevance calculation starts from the output neuron $y$ at the last layer $l_n$ (\ie, $R_y^{l_n}$) until the relevance $R_i^{l_1}$ of the input layer is calculated. At each layer, the sum of the relevance of all neurons is equal to $g_f(x)$. Please refer to~\cite{bach2015pixel} for more details about the backward relevance calculation.



% $$R_j^{(l+1)} = \sum_{i\in(l)} R_{i\leftarrow j}^{(l,l+1)}$$
% $$R_i^{(l)} = \sum_{j\in(l+1)} R_{i\leftarrow j}^{(l,l+1)}$$
% where $R_j^{(l+1)}$ represents the relevance of the neuron $j$ at the layer $l+1$, $R_{i\leftarrow j}^{(l,l+1)}$ represents the relevance of the neuron $i$ at the layer $l$ and the neuron $i$ provides the input to the neuron $j$ at the layer $l+1$.
% The relevance calculation starts from the output neuron at the last layer $l_n$ is $R_y^{(l_n)}=g_f(x)$ until the relevance $R_i^{(1)}$ of the first layer (\ie, the input layer) is calculated. 

As described in Section~\ref{sec:lrp}, the relevance $R_i^{l}$ represents the contribution on the final decision. The larger relevance the relevance  $R_i^{l}$, the more contribution the 
neuron $i$ at the layer $l$. Since the DNN prediction is based on the features extracted and transformed layer-by-layer, we use the critical neurons with large relevance in each layer to represent the internal decision of the DNN. Then we define the critical decision path along all layers of the DNN as follows:

\begin{definition}[Critical Decision Path]\label{def:cdp}
Given an input $x$ and the DNN $f$ consisting of $n$ layers, we define its $\alpha$-Critical Decision Path ($\alpha$-CDP) as a sequence of neurons sets $p=\left\langle s_1,\ldots,s_{n-1}\right\rangle$, where $s_i$ is a set of critical neurons that have the largest relevance values at the layer $l_i$ and
%
$$(\forall j\in s_i. R_j^{l_i}>0) \wedge (\sum_{j\in {s_i}} R_j^{l_i}>\alpha \cdot g_f(x))$$
%
%\qing{i should be j and j should be i? to be consist with the above definitions of $i$ and $j$?}
where $\alpha$ is a parameter that controls the number of the selected critical neurons at each layer. 
\end{definition}


The neuron is \textit{critical} if it provides a positive contribution to the decision (\ie, the positive relevance). We first sort neurons of each layer by the relevance values, and the CDP is composed of the most critical neurons at each layer. As a layer may have multiple critical neurons, we use the parameter $\alpha$ to prioritize the more critical ones. The smaller the $\alpha$, the fewer critical neurons are selected at each layer.
Other neurons that are not selected in the CDP are called \textit{Non-Critical Decision Path (NCDP)}.

We define the width of the CDP as the average ratio of neurons selected at each layer.
It is worth mentioning that, for different inputs, the width of the CDP may be different even with the same value for the parameter $\alpha$.
For each input, we select the CDP that has a large effect on the prediction while the NCDP (\ie, other neurons) has little impact. Furthermore, the width of the CDP (\ie, the selected neurons) should be as small as possible such that it can represent different decision logic accurately. Consider an extreme case like that, we could use all neurons of the network as the CDP, which does not lose any information. However, it cannot distinguish the decision logic between different inputs because all inputs have the same CDP (\ie, the DNN). Our evaluation demonstrated that CDPs with a suitable width could better reveal different predictions, \ie., inputs predicted to be the same class share similar CDPs while inputs predicted to be different classes have different CDPs.

%because the neurons of the CDP are the most critical for the decision. Intuitively, the relevance values of these neurons have a great effect on the calculation of the final output. Our evaluation demonstrated that inputs predicted to be in the same class have similar CDPs (see Section~\ref{sec:eval}).
\subsection{Path Abstraction}\label{sec:pathabstract}
The decision logic of the DNN is determined by the training data, thus we recover its main decision logic that is learned from the training data. Given a classifier $f$ and its training data $T$, we construct the CDP for each sample in $T$, which are used to estimate the learned logic of the DNN roughly.
However, analyzing all CDPs of $T$ may introduce high computational costs especially when the size of $T$ is large. Moreover, some training data may share similar decision behaviors. To reduce the computational cost, we introduce a two-stage method to calculate the abstract CDPs.

\paragraph{Intra-Class Path Clustering} 
The assumption is that, the inputs that are predicted to be the same class, should have similar CDPs because the DNN has similar decisions on these inputs. Thus, our basic idea is to generate representative CDPs, which could characterize the common decision pattern on these inputs.

In particular, suppose the classifier $f$ performs a classification task with a set of classes $Y$, we group the training samples on the predicted class $y\in Y$, \ie, $T_y=\{x\in T | f(x)=y\}$. For each class $y$, although the decision logic on the inputs $T_y$ is similar, they may still have some slight difference. For example, the decision of the yellow cats may be slightly different from the brown cats. %Moreover, some incorrect prediction (\eg, some dogs are predicted as cats) has more different CDPs with the correct ones. 
To capture more fine-grained decision logic in each class $y$, we cluster CDPs of the samples in $T_y$ into $k$ groups. %\qing{Which clustering algorithm is used?}
We apply the $K$-Means clustering algorithm in this paper. Specifically, for each sample, we obtain a vector that represents the status of all neurons of the DNN. If a neuron is included in the CDP, its status is marked as 1 in the vector, otherwise, it is marked as 0. Note that all vectors have the same size such that they can be clustered.
$C_j^y\subseteq T_y$ denotes the training samples in the $j^{th}$ cluster. The samples in the same cluster have more similar decision-making logic than samples in other clusters. 


\paragraph{Path Merging} 
For CDPs in each cluster, we then propose the path abstraction by merging them into an abstract path. Specifically, for $C_j^y$ in the $j^{th}$ cluster, we calculate an abstract CDP $\hat{p} = \left\langle \hat{s}_1,\ldots,\hat{s}_{{n-1}}\right\rangle$ by merging neurons in each layer:
$\forall i\in\{1,\ldots,n-1\}: \hat{s}_i = \bigcup_{x\in C_j^y} s_i^{x}$.
For each neuron $t\in \hat{s_i}$, we calculate its weight as:
$$w_t= \frac{|\{x | x\in C_j^y \wedge t \in s_i^{x}\}|}{|C_j^y|}$$
where $s_i^{x}$ is the set of critical neurons at the layer $i$ in the CDP of the input $x$.

Intuitively, for a set of inputs, the abstract CDP is the union of their critical neurons at each layer. The weight of each neuron $w_t$ represents the ratio of CDPs that the neuron $t$ belongs to. %\qing{Here, the notation confuses me. $j$ is the index for cluster but here $j$ corresponds a neuron?}.
The larger the weight, the more critical this neuron is (\ie, it is critical for more CDPs of training samples in this cluster).
After merging the path, the abstract CDP could be much larger than the CDP of one input. There are some neurons in the abstract CDP, which may have small weight. Statistically, neurons with smaller weights may be less important for interpreting the decision on the set of inputs. Thus, we further introduce the parameter $\beta$ to select the critical neurons whose weights are above the threshold and obtain the abstract CDP $\hat{p}_\beta = \left\langle \hat{s}_{{1,\beta}},\ldots,\hat{s}_{{{n-1},{\beta}}}\right\rangle$, where
$$\hat{s}_{{i,\beta}} = \{t| t\in\hat{s}_i \wedge w_t >\beta \}$$

%The abstract CDPs characterize the expected decision logic of the DNN learned from the training data.
Based on the abstract CDPs, we characterize the decision logic of a DNN as a decision graph, which is similar to the control flow of programs.

\begin{definition}[Decision Graph]
The Decision Graph (DG) of a classifier $f$ is composed of a set of abstract CDPs $G= \{(\hat{p}_{\beta}^{1,1},\ldots,\hat{p}_{\beta}^{1,k}), \ldots, (\hat{p}_{\beta}^{n,1},\ldots,\hat{p}_{\beta}^{n,k})\}$, where $n$ is the number of the classes, $k$ is the number of the clusters for each class and $\hat{p}_{\beta}^{i,j}$ represents the corresponding abstract CDP with regards to the $j^{th}$ cluster of the class $i$.
\end{definition}
\subsection{Neuron Path Coverage}
\label{sec:criteria}
The decision graph represents the main logic of the DNN learned from its training data. 
Given a new input, it is expected that the input could be predicted correctly via the learned decision logic. 
%The fundamental assumption of DL is that the DNN could handle inputs that follow the distribution of the training data while is uncertain on the out-of-distribution inputs.
DL testing aims to identify failed inputs that are possibly caused by triggering either \textit{unknown} logic or \textit{incorrect} logic. Specifically, \textit{unknown} logic means that the CDP of the input has low similarity with abstract CDPs in the DG, \ie, the DNN may not be able to learn the logic with the training data. \textit{Incorrect} logic means that the input exercises the incorrect CDP, \eg, one dog may have a similar CDP with a cat. We propose the path coverage to measure the adequacy of a given test suite. Intuitively, the more paths covered, the more logic explored.

Specifically, inspired by the traditional software testing, we consider the control flow and data flow of the DNN and propose two variants of path-based coverage criteria: the \textit{Structure-based Neuron Path Coverage (SNPC)} and the \textit{Activation-based Neuron Path Coverage (ANPC)}. \textit{SNPC} mainly considers the control flow, \ie, the path structure while \textit{ANPC} considers the data flow, \ie, the neuron outputs in the path. 

Theoretically, like paths in traditional programs, the number of the paths in DNN could be infinite. To mitigate this problem, we follow the strategy~\cite{test:surprise} by calculating the distance and use bucketing to discretize the space of the distance. 

\subsubsection{Structure-based Neuron Path Coverage}
Given an input $x$ with the CDP $p_x$, we first identify the clusters based on the predicted result $f(x)$. Suppose $G_{f(x)} =\{\hat{p}_{\beta}^{f(x),1},\ldots,\hat{p}_{\beta}^{f(x),k}\}$ is the set of abstract paths that are extracted from clusters of the class $f(x)$. We measure the similarity between $p_x$ and each of the abstract paths in $G_{f(x)}$, which represents the difference of the decision behavior of the given input $x$ with the existing abstract paths. Then we divide the similarity into multiple buckets and calculate the coverage, \ie, how many buckets are covered.

Given two paths $p_x$ and $\hat{p}$, we calculate the similarity layer by layer. For a layer $l$, the similarity is:
\begin{equation}\label{sec:jaccard}
    J_{p_x^l,\hat{p}^l}= \frac{s^x_l \cap \hat{s}_l}{s^x_l \cup \hat{s}_l}
\end{equation}
where $s^x_l$ and $\hat{s}_l$ are the neurons in the $l^{th}$ layer of $p_x$ and  $\hat{p}$, respectively.

% The similarity is calculated layer by layer
% cluster $j$ to which $x$ belongs based on $p_x$ and its prediction result $f(x)$. Let $\hat{p}_j$ be the abstract path of the cluster $j$.  with the Jaccard similarity layer by layer. For the layer $l$, the similarity between $p_x$ and  $\hat{p}_j$ is:
% $$J_{p_x^l,\hat{p}_j^l}= \frac{s^x_l \cap \hat{s}_l}{s^x_l \cup \hat{s}_l}$$
% where $s^x_l$ and $\hat{s}_l$ are the neurons in the $l^{th}$ layer of $p_x$ and  $\hat{p}_j$, respectively.

Then we divide the continuous space of the similarity (\ie, [0,1]) into $m$ equal buckets $B=\{b_1,\ldots,b_m\}$. For an input $x$ and a target abstract path $\hat{p}$, the covered bucket at layer $l$ is denoted as:
$$b_{x, \hat{p}}^l = b_i \text{ if } J_{p_x^l,\hat{p}^l}\in (\frac{i-1}{m}, \frac{i}{m}]$$

 
 
 
%  Given two sets of neurons $S_1$ and $S_2$, we calculate its distance with the Jaccard similarity:
% $$D_{S_1,S_2}=\frac{S_1 \cap S_2}{S_1 \cup S_2}$$
% Specifically, we use $D_{p_1^l, p_2^l}$ to represent the layer similarity at the layer $l$ between $p_1$ and $p_2$.
% % we use $D_{p_1, p_2}$ to represent the path similarity between two paths $p_1$ and $p_2$, and use $D_{p_1^l, p_2^l}$ to represent the layer similarity at the layer $l$ between $p_1$ and $p_2$.
% Then we divide the continuous space of the distance (\ie, [0,1]) into $m$ equal buckets $B=\{b_1,\ldots,b_m\}$.
% Given an input $x$ with the CDP $p_x$ and the target path $p$, the layer similarity can fall into the bucket:
% %$$b_{x, p} = b_i \text{ if } D_{p_x,p}\in (\frac{i-1}{m}, \frac{i}{m}]$$
% $$b_{x, p}^l = b_i \text{ if } D_{p_x^l,p^l}\in (\frac{i-1}{m}, \frac{i}{m}]$$

%Given a classifier $f$, its DG $G= \{(\hat{p}_{\beta}^{1,1},\ldots,\hat{p}_{\beta}^{1,k}), \ldots, (\hat{p}_{\beta}^{n,1},\ldots,\hat{p}_{\beta}^{n,k})\}$ and 
Given a test suite $X$, we define the Structure-based Neuron Path Coverage as follows:
%$$NPC(X)=\frac{|\{b_{x,p} | \forall x\in X, \forall p \in G_{f(x)} |}{n*k*m}$$
\begin{equation}
    SNPC(X)=\frac{|\{b_{x,\hat{p}}^l | \forall x\in X, \forall \hat{p} \in G_{f(x)}, \forall l \in f\}|}{n\cdot k \cdot |\hat{p}| \cdot m}
\end{equation}
 where $\hat{p}$ is the corresponding abstract CDP, $|\hat{p}|$ is the total number of layers, 
 $n$ is the number of the total classes, $k$ is the number of clusters in the class $f(x)$ and $m$ is the number of buckets. %$G_{f(x)} =\{\hat{p}_{\beta}^{f(x),1},\ldots,\hat{p}_{\beta}^{f(x),k}\}$ is the set of abstract paths that are extracted from clusters of the class $f(x)$.

\revise{
Specifically, for each layer of the abstract path, we divide the neuron similarity [0, 1] (\ie, Jaccard similarity) between two layers into $m$ buckets. Finally, there are a total of $n \cdot k \cdot |\hat{p}| \cdot m$ buckets, where $n\cdot k $ is the total number of abstract CDPs and $|\hat{p}| $ is the number of layers. SNPC calculates how many buckets can be covered by a test suite $X$.
For a test case $x\in X$ and a layer $l$, we calculate the layer similarity between the CDP of $x$ and the corresponding abstract CDP $\hat{p}$. The similarity falls into a specific bucket $b_{x, \hat{p}}^l$. We identify all buckets covered by the test suite $X$, \ie, $\{b_{x,\hat{p}}^l | \forall x\in X, \forall \hat{p} \in G_{f(x)}, \forall l \in f\}$, and calculate the coverage.
}


The higher the coverage criteria, the more diverse logic the DNN has been explored. However, \textit{SNPC} only considers the control flow, which might be coarse in some cases. To be more fine-grained, we therefore propose another variant of path coverage that adopts the concrete activation values of neurons in the path (\ie, data flow).

\subsubsection{Activation-based Neuron Path Coverage} 
In SNPC, we adopt the Jaccard similarity to calculate the structural similarity between the CDP of the input $x$ and the abstract CDP of a cluster. To be more fine-grained, we consider the data flow of the CDP, \ie, the activation values of neurons in the CDP and calculate the distance between the values of two CDPs. Specifically, given an input $x$ and a cluster $j$, we first select the closest training sample $x'$ from the cluster $j$, which has highest similarity with $x$: $$x' = \argmax_{x'\in C^{f(x)}_j} J_{p_x, p_{x'}} $$ where $J_{p_x, p_{x'}}$ is the Jaccard similarity between CDPs of $x$ and $x'$.
Then, we calculate the distance between the activation values of $x$ and $x'$ along the abstract CDP in the cluster. Intuitively, the larger the distance, the more different decision behaviors are triggered by the new input $x$, \ie, compared with the samples in cluster $j$, more behaviors are covered by the new input. For the input $x$, we use $A(x, \hat{p}^l)$ to denote the activation values of neurons in the $l^{th}$ layer of the abstract path $\hat{p}$. The distance at the $l^{th}$ layer between $x$ and $x'$ is defined as:
$$D^l_{x,x'}=||A(x, \hat{p}^l) - A(x', \hat{p}^l)||$$

Similar to~\cite{test:surprise}, we introduce an upper bound $U$ and divides the distance $[0,U]$ into $m$ buckets: $B=\{b_1,\ldots,b_m\}$. Given an input $x$ and an abstract path $\hat{p}$ in the corresponding cluster, we define  $d_{x, \hat{p}}^l$ as the covered bucket, \ie, the layer distance $D^l_{x,x'}$ falls into a bucket: $$d_{x, \hat{p}}^l = b_i \text{ if } D^l_{x,x'} \in (U \cdot  \frac{i-1}{m}, U \cdot  \frac{i}{m}]$$

Given a test suite $X$, we define the Activation-based Neuron Path Coverage (ANPC) as:
\begin{equation} ANPC(X)=\frac{|\{d_{x,\hat{p}}^l | \forall x\in X, \forall \hat{p} \in G_{f(x)}, \forall l \in f\}|}{n\cdot k\cdot |\hat{p}|\cdot m}
\end{equation}

From the definitions, we can see that the key difference between SNPC and ANPC is that SNPC calculates the distance (\ie, $b_{x,\hat{p}_j}^l$) based on the path structure similarity while ANPC calculates the distance (\ie, $d_{x,\hat{p}}^l$) based on the neuron activation distance. With the coverage criteria, we could measure the adequacy of the test suite with regards to the decision behaviors.
\revise{
\subsubsection{Hyperparameter Tuning}
In the two coverage criteria, we have three hyperparameters, \ie, $\alpha$, $\beta$ and $k$, which determine the precision of the (abstract) CDPs  with regards to representing the decision logic. To adopt the proposed coverage criteria in DL testing, the hyperparameter tuning is required. We propose a strategy to evaluate the precision of the CDPs (under a set of hyperparameters) on representing the decision logic as follows:

\begin{enumerate}
    \item For each training data, we extract its CDP and the NCDP. The expectation is that the CDP has large impact on the decision of the data while the NCDP has less impact on the decision. Moreover, the width of the CDP is as small as possible such that only critical neurons are selected. Specifically, we respectively dropout the outputs of neurons (\ie, mask the results as zero) in the CDP and the NCDP, and evaluate whether the prediction result is changed (\ie, inconsistent). We evaluate the inconsistency rate on all training data on some hyperparameters and select the best ones that satisfies our assumption.
    \item Similarly, we evaluate the precision of abstract CDPs. For the abstract CDP of a cluster, we calculate the inconsistency rate on all training data of the cluster. For each data, we dropout the same neurons that belong to the abstract CDP. The inconsistency rate is expected to be high by masking the neurons of the abstract CDP and low by masking the neurons of the abstract NCDP.
\end{enumerate}
}


% The distance between two paths $p_1$ and $p_2$ is calculated by the Jaccard similarity:
% $$D_{p_1,p_2}=\frac{S_{p_1} \cap S_{p_2}}{S_{p_1} \cup S_{p_2}}$$
% where $S_p$ means all neurons in the path $p$, \ie, the union of neurons at each layer.
% We divide the continuous space of the distance (\ie, [0,1]) into $m$ equal buckets $B=\{b_1,\ldots,b_m\}$, given a input $x$ and a target path $p$, we calculate the covered bucket of $x$ with regards to $p$ as: 
% $$b_{x, p} = b_i \text{ if } D_{p_x,p}\in (\frac{i-1}{m}, \frac{i}{m}]$$


% Based on the bucketing, we propose two coverage criteria: \textit{Intra-class Neuron Path Coverage (Intra-NPC)} and \textit{Inter-class Neuron Path Coverage (Inter-NPC)}. Given a new test input and its predicted class, \textit{Intra-NPC} only considers the relationship with paths in the predicted class while\textit{ Inter-NPC} considers the relationship with paths in all classes.
% Given a classifier $f$, its DG $G= \{(\hat{p}_{\beta}^{1,1},\ldots,\hat{p}_{\beta}^{1,k}), \ldots, (\hat{p}_{\beta}^{n,1},\ldots,\hat{p}_{\beta}^{n,k})\}$ and a test suite $X$, we define the \textit{Intra-NPC} and \textit{Inter-NPC} as follows:
% $$Intra-NPC(X)=\frac{|\{b_{x,p} | \forall x\in X, \forall p \in G_{f(x)} |}{n*k*m}$$
% $$Inter-NPC(X)=\frac{|\{b_{x,p} | \forall x\in X, \forall p \in G_a\}|}{n*k*m}$$
% where $n$ is the number of the total classes, $k$ is the number of clusters in each class and $m$ is the number of the buckets, $G_{f(x)} =\{\hat{p}_{\beta}^{f(x),1},\ldots,\hat{p}_{\beta}^{f(x),k}\}$ is the set of abstract paths that are extracted from clusters of the class $f(x)$ and $G_a$ is the set of all abstract paths in $G$.


==> sections-old/eval_.tex <==
\section{Evaluation}\label{sec:eval}
To evaluate effectiveness of our approach, we implemented $NPC$ in Python based on the PyTorch framework. The objectives of the evaluation are to demonstrate that our approach is \textit{interpretable} and \textit{effective}. As we claimed in Section~\ref{sec:motivation}, one better coverage criterion should be interpretatble, thus we first evaluate the usefulness of the CDP in interpreting the internal decision of the DNN (\textbf{RQ1} and \textbf{RQ2}). Motivated by the recent works~\cite{ncmislead,nerualmisled,dong2019limited}  that show the limitation of the existing coverage criteria, we then evaluate the effectiveness of NPC, \ie, whether there is correlation on defect detection and output impartiality (\textbf{RQ3} and \textbf{RQ4}).
Specifically,
our experiments are designed to answer the following research questions:
\begin{itemize}
    \item \textbf{RQ1}: How does the CDP affect the decision of the DNN?
    \item \textbf{RQ2}: How accurate is the abstract CDP in revealing internal decisions?
    \item \textbf{RQ3}: Is NPC correlated to the defect detection?
     \item \textbf{RQ4}: Is NPC correlated to the output impartiality?
\end{itemize}


% \subsection{Research Questions}
% \begin{itemize}
%     \item \textbf{RQ1:}How accurate is the path extracted from the neural network?  
    
%     1) Single Image - Mask
%       path width: 1\%, 3\%, 5\%, 10\%
%       maks intervals: [0-1], [1-2],[2-3],[3-4]... [9-10],    10 
       
%       1\%
%     2) Mutiple images - Abstract Path - Mask - Effect
%       path width: 1\%   %, 3\%, 5\%, 10\%
%       maks intervals: [0-1], [1-2],[2-3],[3-4]... [9-10],    10 
%       cluster num: 1, 3, 5, 8 10
      
%      \item \textbf{RQ2:}
%      How useful the path in interpreting neural networks?
%      -- Cluster and Show images
%      1) visulize images in each cluster and calculate acc in each cluster.
%      2) the similarity in intra-class is less than inter-class?
%      intra-class in one cluster: average distance 
%      intra-class between two clusters: average distance
%      inter-class between two clusters: ...
     
     
%      3) the adversarial example vs original input?   0-1/4, 1/4-2/4, 2/4-3/4, 3/4-4/4, whole
%       4) Distinguish different adversarial attacks? original,  CW, FGSM, PGD  (1/4, 2/4, 3/4, 4/4)
%       original -> cw1, cw2, similarity 
     
%      c(2,4)
%      ori: cw
%      ori: pgd
%      ori: fgsm
%      cw: pgd
%      pgd1:Pgd2
    
      
     
%      \item \textbf{RQ3:}
%      Is the path coverage correlated to the defect detection?
     
%      -- prepare some test suites and calculate the correlation
%      \item \textbf{RQ4:}
%      Can the path coverage distinguish same-size test sets of natural examples with different levels of misclassification rates?
     
%      -- prepare some data included different number of natural errors
%      \item \textbf{RQ5:}
%      Is path coverage correlated to the output Impartiality?
     
%      --prepare some test suites and calculate the correlation
     
% \end{itemize}
\subsection{Datasets and DNNs}
We selected three widely used datasets in the image classification domain and trained four models with competitive test accuracy, which are widely used in the previous works~\cite{ma2018deepgauge,test:surprise,pei2017deepxplore}.

\begin{itemize}
    \item \textbf{MNIST}~\cite{mnist} is for handwritten digit image recognition (\ie, handwritten digits from $0$ to $9$), containing $60,000$ training data and $10,000$ test data. Each MNIST image is a single-channel of size $28 \times 28 \times 1$.
    We select the five layer Convolutional Neural Network~\cite{test:surprise} (named \emph{SADL-1}) and achieve an accuracy of 99.1\%.
    \item \textbf{CIFAR-10}~\cite{cifar} is a collection of images for general-purpose image classification, including $50,000$ training data and $10,000$ test data in $10$ different classes~(\eg, airplanes, cars, birds, and cats). Each CIFAR-10 image is three-channel of size $32 \times 32 \times 3$. We select two models, \ie, the 12-layer Convolutional Neural Network~\cite{test:surprise} (named \emph{SADL-2}) and VGG16, which achieved the accuracy of 90.36\% and 89.17\%, respectively.
    \item \textbf{SVHN}~\cite{netzer2011reading} dataset is obtained from house numbers in Google Street View images, including 73,257 training data and 26,032 test data. Each MNIST image is a single-channel of size $32 \times 32 \times 1$. We select the model ResNet-18 that has an accuracy of 96.27\%.

% \noindent\textbf{ImageNet.} To further demonstrate that {\tool} scales to practical-sized dataset and DNN models, we also select ImageNet, which is a large-scale visual recognition challenge~(ILSVRC) dataset for general-purpose image classification. The complexity of ImageNet is characterized by a large number of training data~(\ie, over one million) and test data~(\ie, 50,000), as well as large data points, each of which is of size $224 \times 224 \times 3$ ($\sim 50$x dimensionality of CIFAR-10).
\end{itemize}
\subsection{Baselines}
For RQ3 and RQ4, we select the state-of-the-art coverage criteria as the baselines for the comparison.
\begin{itemize}
    \item \textbf{Neuron Coverage (NC)}~\cite{pei2017deepxplore}, which measures the ratio of activated neurons of a DNN by a test suite. %We configure neuron coverage with different thresholds, \ie, 0.2, 0.5, 0.75.
   \item \textbf{$k$-Multisection Neuron Coverage (KMNC)}~\cite{ma2018deepgauge}, which divides the the range of the neuron outputs (obtained from training data) into $k$ buckets. Then, KMNC measures the ratio of buckets of all neurons covered by a test suite.
    % For a prediction, one section in each neuron will be covered. KMNC is a more fine-grained criterion that represents which sections of neurons are covered.
    \item \textbf{Neuron Boundary Coverage (NBC)}~\cite{ma2018deepgauge}, which focuses on the corner-case buckets of the output of each neuron, and measures the ratio of corner-case buckets covered by a test suite. 
    \item \textbf{Likelihood-based Surprise Coverage (LSC)}~\cite{test:surprise}, that measures the coverage based on the likelihood-based surprise, \ie, how diverse (surprise) is the test suite,
    \item \textbf{Distance-based Surprise Coverage (DSC)}~\cite{test:surprise}, similarly, which measures the coverage based on the distance-based surprise.
\end{itemize}
For NC, we set the threshold as 0, 0.2, 0.5 and 0.75 following~\cite{ncmislead}. For KMNC and NBC, we follow the configuration~\cite{ma2018deepgauge,test:deephunter} and set the $k$ value as 1,000 and 10. For LSC and DSC, we follow the configuration~\cite{test:surprise} by setting the number of buckets as 1,000, the upper bound 2000 and 2.0 for LSC and DSC, respectively. For the layer selection, we select the same layer in SADL-1 and SADL-2, which is used in~\cite{test:surprise}. For VGG16, we select the last layer. For NPC and LNPC, we set the number of buckets as 100.

\subsection{RQ1: Relationship between CDP and the DNN Decision}

\begin{table*}[!t]
    \centering
    \caption{The average width (\%) and inconsistency rate (\%) after masking neurons in the CDP and NCDP}
    % Preview source code for paragraph 0
% Preview source code for paragraph 0

% Preview source code for paragraph 0
% Preview source code for paragraph 0

\begin{tabular}{cc|ccc|ccc|ccc|ccc}
\toprule 
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{$\alpha=0.7$} & \multicolumn{3}{c|}{$\alpha=0.8$} & \multicolumn{3}{c|}{$\alpha=0.9$} & \multicolumn{3}{c}{$\alpha=1$}\tabularnewline
% \cline{3-14}
 &  & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC\tabularnewline
\midrule 
\midrule 
MNIST & SADL-1 &  9.3 & 89.3 & 9.6 & \textbf{12.8} & \textbf{95.8} & \textbf{1.9} & 17.2 & 97 & 0 & 33.3 & 98.9 & 1.8\tabularnewline
% \cline{2-14} \cline{3-14} \cline{4-14} \cline{5-14} \cline{6-14} \cline{7-14} \cline{8-14} \cline{9-14} \cline{10-14} \cline{11-14} \cline{12-14} \cline{13-14} \cline{14-14} 
\midrule
\multirow{2}{*}{CIFAR} & SADL-2 & \textbf{20.9} & \textbf{100} & \textbf{0} & 27.2 & 100 & 0 & 36.3 & 100 & 0 & 63.4 & 100 & 0\tabularnewline
 & VGG16 & 10.2 & 100 & 12.1 & {13.3} & {100} & {1.5} & \textbf{17.9}& \textbf{100} & \textbf{0.1} & 33.8 & 100 & 0\tabularnewline
% \cline{2-14} \cline{3-14} \cline{4-14} \cline{5-14} \cline{6-14} \cline{7-14} \cline{8-14} \cline{9-14} \cline{10-14} \cline{11-14} \cline{12-14} \cline{13-14} \cline{14-14} 
\midrule
SVHN & ResNet-18 & 39.7 & 99.1 & 13.7 & \textbf{49.9} &\textbf{ 99.9 }&\textbf{ 3.1} & 63.7 & 100 & 0.5 & 94.6 & 99.4 & 0\tabularnewline
\bottomrule 
\end{tabular}

    \label{tab:singleinc}
\end{table*}

\textbf{Setup.} 
To evaluate whether the critical decision path (CDP) has a critical impact in the decision of the DNN, we dropout outputs of neurons in the CDP (\ie, mask them as zero) and check whether the predicted result is inconsistent with the original result. Intuitively, we say the CDP is ore accurate to reveal the decision if 1) the predicted output is largely affected after the neurons of the CDP are masked and 2) the predicted output is less affected after neurons in the non-critical decision path (NCDP) are masked. We extract CDPs for all training data and calculate the inconsistency rate after masking neurons in their CDPs and the corresponding NCDPs, respectively. 

Table~\ref{tab:singleinc} shows the average inconsistency rate by masking neurons in the CDPs/NCDPs of all training data. To extract the path, we configure the parameter $\alpha$ (see Definition~\ref{def:cdp}) with different values, \ie, 0.8, 0.9 and 1. Under each configuration, we show the average width of the CDP (Column \textit{Wid.}), which is the average ratio of neurons at each layer of the CDP, the inconsistency rate after masking CDP (Column \textit{Inc.C}) and masking NCDP (Column \textit{Inc.NC}).


The results show that the width of the CDP increases as the parameter $\alpha$ increases. For example, when $\alpha$ is 0.8, the average width of VGG16 is 13.3\%, indicating that 13.3\% critical neurons are selected at each layer. When $\alpha$ is 1, the width becomes much larger (\ie, 33.8\%).
Furthermore, we found that almost all predicted results are changed when the CDPs are masking (\eg, for SADL-2 and VGG16, the inconsistency rate is 100\% for all configuration),
%for models in MNIST and CIFAR-10), 
which demonstrates that the CDP is very important for the decision. Conversely, when we mask other neurons that are not in the CDP (\ie, the NCDP), the inconsistency is very low (0\% to 3\%). In particular, when $\alpha$ is small, the width is small (\ie, less neurons are selected) and the performance is relatively low. For example, when $\alpha$ is 0.7, the inconsistency rate of masking CDP in SADL-1 is 89.3\%, which is lower than 98.9\% ($\alpha=1$);
The inconsistency rate of masking NCDP in ResNet-18 is much higher (13.7\%) than other configurations, which show that there are some critical neurons (in NCDP) which are missed.
%It is a trade-off between the width of the CDP and its representation on the decision logic. 

\begin{table}
\centering
\caption{The average similarity in SADL-1}
\begin{tabular}{ccccc}
\toprule
 & $\alpha=0.7$ & $\alpha=0.8$ & $\alpha=0.9$ & $\alpha=1$\tabularnewline
\midrule 
\midrule
Width & 9.3\% & 12.8\% & 17.2\% & 33.3\%\tabularnewline
\midrule 
Intra-Class & 0.347 & 0.391 & 0.453 & 0.563\tabularnewline
Inter-Class & 0.577 & 0.625 & 0.676 & 0.745\tabularnewline
\bottomrule
\end{tabular}
\label{tab:distance}
\end{table}
The width of the CDP may affect its accuracy 
in representing the decision logic. If the width is too large, the CDP contains some non-critical neurons that may also be included in other CDP, making it hard to distinguish them. Table~\ref{tab:distance} shows the average similarity between two CDPs in the same class (\ie, Column \textit{Intra-Class}) and in different classes (\ie, Column \textit{Inter-Class}). The results show that the average similarity increases as the increase of the width, which further demonstrates that, if the CDP is too wide, it is not accurate to show the decision difference on two inputs. Similar trends are also shown in the results of other models~\cite{deepnpc}. If the width of the CDP is too small, then it may miss some critical neurons (see Table~\ref{tab:singleinc}). Finally, in the following experiments, we configure $\alpha$ as 0.8, 0.7, 0.9 and 0.8 for SADL-1, SADL-2, VGG16 and ResNet-18, respectively.

%or too small, the CDP may include more non-critical neurons or miss more critical neurons, making it hard to distinguish the logic of two inputs well. Fig.~\ref{XXX}...
%Our goal is to select the CDP, which has smaller width (\ie, the CDP is representative) and could can represent the decision logic accurately, \ie, the CDP is important for decision-making and the corresponding NCDP is not important for decision-making. 


%\textbf{Performance.} The average time spent for extracting the CDP of an input is \fei{}, \fei{}, \fei{} and \fei{}, respectively. 


\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ1:}} 
The CDPs are critical for the prediction while the NCDPs are non-critical, which indicate that the CDPs could represent the internal decision logic of the DNN.
%\fei{In addition, the width of the CDP is sensitive for representing the decision of the DNN.}
%With path abstraction, we could reduce the total number of CDPs. The abstract CDP could become narrow (\ie, smaller width) while the performance is still competitive. 
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}

%$\alpha=0.9$ because it could achieve similar accuracy with $\alpha=1$, but the width of CDPs is much smaller.
%and the inconsistency rate of masking NCDP in VGG16 (22\%) is much higher than other two configurations.




% Specifically, we evaluate the accuracy of the 
% single CDP and the abstract CDP. For the single CDP, we extract CDPs for 10,000 test data in each dataset, and calculate the inconsistency rate, \ie, how many test data whose result will be inconsistent by masking neurons in their CDPs and the corresponding NCDPs, respectively. 

%For abstract CDPs in the decision graph, some training samples (in the cluster of a class) share the same abstract CDP, we mask the neurons of this abstract CDP and check the inconsistency rate of all training samples in this cluster. Finally, we calculate the average inconsistency rate of all clusters in different classes.

\begin{table*}[!t]
    \centering
    % Preview source code for paragraph 0

    \caption{The average width and inconsistency rate (\%) after masking neurons in the abstract CDP and NCDP}
% Preview source code for paragraph 0

\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\#Cluster} & \multicolumn{3}{c|}{SADL-1 ($\beta=0.8$)} & \multicolumn{3}{c|}{SADL-2 ($\beta=0.9$)} & \multicolumn{3}{c|}{VGG16 ($\beta=0.9$)} & \multicolumn{3}{c}{ResNet-18 ($\beta=0.99$)}\tabularnewline
% \cline{2-13} 
 & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC\tabularnewline
\midrule
\midrule 


1 & 12.5 & 78.8 & 29.9 & 4.1&	90.9 &	2.4
%3.3 & 82.1 & 9.7 
& 7.9 & 100 & 10.1 &10.8  & 90.7  &6.9 \tabularnewline
4 & \textbf{14.6} & \textbf{94.1} &\textbf{ 3.9 }&
%5.1 & 94.3 & 5.6 
4.8	& 95.3	& 2 & 8.4 & 100 & 9.2 & 
\textbf{12.7} & \textbf{95.6 }& \textbf{3.7} \tabularnewline
7 & 14.6 & 92.5 & 2.9 & 
%5.9 & \textbf{98.7 }& \textbf{0} 
\textbf{5.4}	& \textbf{98.2}&\textbf{	1.6}& \textbf{8.7} & \textbf{100 }& \textbf{4.9} & 
13.3 &95.1  &3.7 \tabularnewline
\bottomrule 
\end{tabular}


    \label{tab:abstractp}
\end{table*}
%\paragraph{Accuracy of Single CDPs}

\subsection{RQ2: Effectiveness of Path Abstraction}
\textbf{Setup.} 
We firstly evaluate whether the abstract path (extracted from one cluster) is critical for the prediction of inputs in the corresponding cluster. Similar with RQ1, we mask the abstract CDP/NCDP and see the average inconsistency rate of these inputs. Then we evaluate whether the path abstraction could merge similar decision logic together by measuring the distance between clusters and within clusters.

\subsubsection{Impact on prediction}
For the path abstraction of each DNN, we set a total of 9 configurations with different parameters $(k, \beta)$, where $k$ is the number of the clusters in each class and $\beta$ is the threshold to select neurons with higher weights. Due to the space limit, for each DNN, we only show part of the results by selecting its better parameter $\beta$ in Table~\ref{tab:abstractp}.
The complete results could be found in our website~\cite{deepnpc}.  The first column \textit{Cluster.} shows the parameter $k$ (\ie, the number of the clusters). Note that, when $k=1$, the abstract CDP is extracted by merging CDPs of all inputs that are predicted as the class.

The results show that, with the increase of the number of clusters, the width tens to be larger under the same threshold $\beta$ (see Column \textit{Wid.}), which indicates that the average weight of neurons is larger (\ie, CDPs in each cluster share more common neurons); The inconsistency rate after masking neurons of the abstract CDP tends to be larger (see Column \textit{Inc.C}), the inconsistency rate after masking neurons of the abstract NCDP becomes smaller (see Column \textit{Inc.NC}). The reason is that more fine-grained clustering (\ie, more clusters) could merge the similar CDPs together, by which the abstract CDP is more \textit{stable} (larger average weights) and \textit{accurate} (higher inconsistency rate after masking CDPs and lower inconsistency rate after masking NCDPs). The results demonstrate the usefulness of clustering and merging.

Compared with the results on single CDPs (Table~\ref{tab:singleinc}), we found that the abstract path could still achieve competitive performance and even better than single CDPs on some models. 
For example, on SADL-2, the inconsistency rate of CDP and NCDP are 98.2\% and 0\% ($k=7$), which are close to results of single CDPs (\ie, 100\% and 0\%) and the width is much smaller (\eg, 5.9\% for abstract CDPs and 26.2\% for single CDPs). For ResNet-18, with the statistical analysis in the cluster, we could select more accurate CDPs (\eg, the average width of the abstract CDPs and the single CDPs is 12.7\% and 39.7\%).
Finally, we select 4, 7, 7, 4 as the number of clusters for SADL-1, SADL-2, VGG16 and ResNet-18, respectively (the bold numbers).
%Based on the results in Table~\ref{sec:pathabstract}, 
%For VGG16, when $k=7$, the results are better than results of single CDPs with $\alpha=0.8$. Specifically, the abstract CDPs are more accurate, \ie, they have the same  inconsistency rate on CDPs (100\%) but smaller on NCDPs (4.9\% and 22.4\%). 
%Moreover, based on the statistical analysis in the cluster, path abstraction could help further reduce the width of the abstract CDPs. For example, for the SADL-2, we could  is 
%abstract CDPs with small width and high accuracy.
\begin{figure}
    \centering
     \includegraphics[width=0.95\linewidth]{pics/show_case.pdf}
    \caption{Inputs sampled from clusters in the class 4 and 5}
    \label{fig:clustervis}
\end{figure}
\subsubsection{Decision Revealing}
% Preview source code for paragraph 0
Table~\ref{tab:clustersim} shows the results on the average similarity with and without clustering. Column \textit{\#Clus.} shows the number of clusters configured for each model.  Column \textit{\#Intra\_Cla.} shows the average similarity between CDPs that are in the same class (\ie, the intra-class similarity). Column \textit{\#Inter\_Cla.} shows the average similarity between CDPs that belong to different classes (\ie, the inter-class similarity). After the clustering, we show the average similarity between CDPs in the same cluster (\ie, intra-cluster similarity shown in Column \textit{\#Intra\_Clus.}) and the average similarity between CDPs in different clusters of the \emph{same} class (\ie, inter-cluster similarity shown in Column \textit{\#Inter\_Clus.}). Note that inter-cluster similarity only compares clusters that are in the same class

Comparing the results between intra-class similarity (without clustering) and intra-cluster similarity (with clustering), we found that the average similarity increases (\eg, from 0.625 to 0.708 in SADL-1). In particularly, we found that, in the same class, inter-cluster similarity is much smaller than intra-cluster similarity although the two clusters belong to the same class (\eg, 0.708 for intra-cluster and 0.381 for inter-cluster).
Moreover, we found that, the inter-cluster similarity is even close to the inter-class similarity. The results demonstrate that samples in the same class could have very different decision logic (\eg, the black dogs and white dogs may be different). By the path abstraction, we generate the fine-grained CDPs which could distinguish such difference well.

Fig.~\ref{fig:clustervis} shows inputs whose CDPs are clustered into different groups (on SADL-1). Each row represents one cluster.
We can observe that, from human's perception, the inputs in the same cluster look very similar. For example, the number 4 looks similar with 9 in the fourth cluster and the number 5 tends to lie down in the first cluster. The results further show that the inputs trigger the similar decision logic could be grouped into one cluster based on the extracted CDPs.

\begin{table}[!t]
    \centering
    
    \caption{The average similarity with and without clustering}
\begin{tabular}{cccccc}
\toprule 
Model & \#Clus. & Intra\_Cla. & Inter\_Cla. & Intra\_Clus. & Inter\_Clus.\tabularnewline
\midrule 
\midrule 
SADL-1 & 4 & 0.625 & 0.391 & 0.708 & 0.381\tabularnewline
SADL-2 & 7 & 0.497 & 0.230 & 0.524 & 0.260\tabularnewline
VGG & 7 & 0.671 & 0.321 & 0.703 & 0.316\tabularnewline
%  ResNet-18&4&0.623 & 0.644 & 0.567 & 0.566\tabularnewline
\bottomrule 
\end{tabular}
    \label{tab:clustersim}
\end{table}



\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ2:}} 
With the statistical analysis in each cluster, the abstract CDP is still critical for predicting all inputs in a cluster. Moreover, the abstract CDP is sensitive to reveal different decision logic. Inputs in the same cluster have similar decision and inputs in different clusters of the same class have different decision.
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}
\vspace{-.1in}
\subsection{RQ3: Sensitivity with Defect Detection}
\textbf{Setup.} Motivated by~\cite{ncmislead,nerualmisled}, this experiment evaluates the effectiveness in detecting defects including the natural errors and the adversarial examples. We follow the similar design in~\cite{nerualmisled}: First, we randomly select 1,000 benign samples (denoted as $s_b$) from the test data. 
Then, we construct several test suites by replacing a small number of samples of $s_b$ (\ie, 1\%, 3\%, 5\%, 10\%, 15\%, 20\%) with the same number of errors such that they have the same size. Specifically, for natural errors, we select inputs from test data, that are predicted incorrectly. For adversarial examples, we adopt the PGD attack~\cite{madry2018towards} to generate 
a large number of adversarial examples, some of which are then randomly selected. Finally, for each DNN, we generate 7 test suites including 
different numbers of errors and calculate their coverage with different criteria. 
%The expectation is that the code coverage should be sensitive in different numbers of errors.

Fig.~\ref{fig:coveragechange} shows the results on the test suites including different number of errors. To conduct the comparison between different approaches, all the coverage is normalized to [-1,1]. The first row shows the results on natural errors (\emph{Nat.}) and the second row shows the results on adversarial examples (\emph{AE}). The horizontal axis shows the percentage of errors while the vertical axis shows the normalized coverage. 
Consider the natural errors at the first row, we could find that, as the number of natural errors increases, NPC and LNPC increase in all three models. It is because new decision logic is triggered by the natural errors and our method is sensitive in such new decision behavior. Similarly, DSC is also increasing with the increase of errors. LSC increases on VGG16 but it is not accurate in SADL-1 (\eg, the coverage does not change after adding 5\% and 10\% errors).
Note that, LSC does not change on SADL-2 because the Surprise Adequacy value is NaN and Inf in almost all layers. Compared with LSC and DSC, our method considers the relationship between all layers and
does not rely on the selection of layers. 


%However, the existing structural coverage criteria are not sensitive in the new errors. 

For others, NC with all four thresholds (denoted as NC-ALL) does not change any more (\ie, $y$=0), which show that NC is too coarse-grained. KMNC is in a decreasing trend, which seems to be aligned in its design, \ie, they mainly cover the major function of DNNs. Hence, when some benign samples are replaced with errors that may cover corner cases, the coverage of major region decreases. 
%LSC and DS shows a certain degree of increasing trend on SADL-1 and VGG16 but does not change on SADL-2. 

Consider adversarial examples at the second row, we observed that the coverage usually decreases as the number of the adversarial examples increases. On SADL-2 and VGG16, we could still observe the similar trend with existing coverage criteria (\eg, the coverage increases firstly and then decreases). Surprisingly, on ASDL-1, we achieved totally different results, \ie, the coverage decreases as the adversarial examples are adding.   
We made a deep analysis and found the following two possible reasons, 1) although the number of adversarial examples increases, many of them are more close to the corresponding abstract CDP than the natural samples (\ie, triggered the known logic). It is because the PGD attack adopts the gradient-based that tends to generate inputs towards one direction, decreasing the diversity of inputs. 2) many adversarial examples are predicted into one specific class (\ie, the prediction is biased to one class). 
%trigger similar decision logic. Meanwhile, we removed the same number of benign samples, which actually trigger more diverse decision than the inserted adversarial samples.  
From the results of natural errors and adversarial examples, we could conclude that natural errors introduce more information (\ie, trigger more different decision) than the adversarial examples.
%However, we could still found that there are some similar trend between our coverage and the existing criteria. For example, on SADL-2, similar with KMNC and NBC, the coverage of NPC and LNPC 
%is decreased to the minimum when 20\% adversarial examples are introduced. On VGG16, similar with KMNC, NBC and LSC, the coverage of LNPC increases when the number of adversarial examples increase by 1\%, 3\%, 5\%, 10\% and 15\% but decrease after 20\% adversarial examples are introduced in the test suite.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{pics/defecttrend.pdf}
    \caption{Coverage change on test suits including different number of errors.}
    \label{fig:coveragechange}
\end{figure}


% or they are similar with other benign samples in the test suite. Meanwhile, we removed the same number of benign samples, which actually trigger more diverse decisions than the inserted adversarial samples. Thus, our coverage may decrease when more errors are introduced.

%The results show that natural errors could introduce more information (\ie, trigger different decision) than the adversarial examples.




\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ3:}} 
NPC and LNPC are sensitive with the natural errors. The further analysis show that adversarial samples trigger limited decision logic than the natural errors.
%and the removed benign samples.
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}
\vspace{-.1in}
\subsection{RQ4: Correlation with Output Impartiality}
\textbf{Setup.} As described in~\cite{ncmislead,test:deephunter,alshahwan2014coverage}, the test data or errors should be diverse. A test suite containing only one category of samples is not enough to reveal defects of the DNN. The tests in a test suites should exercise more diverse output behavior with different decision. The coverage criteria should be aware of the prediction bias~\cite{ncmislead}.
We follow the similar setting in~\cite{ncmislead} and use the same tool to generate 386 test suites (48, 171 and 167 for SADL-1, SADL-2 and VGG16), which have different levels of prediction bias. Based on the coverage and output diversity of test suites, we calculate its correlation~\cite{ncmislead}.


\felix{missing figure and table refs below:}

Figure~\ref{} visualizes the relationship between NPC/LNPC and the output impartiality and Table~\ref{} shows the correlation on different models. The results demonstrated that the proposed path coverage is strongly correlated with the output impartiality. It is easy to understand because we recover the decision logic (\ie, the abstract CDPs) for the prediction of each class. Then NPC and LNPC measure how different the CDPs of test suites with the abstract CDPs. Thus, a test suite including more diverse outputs will trigger more diverse decision logic with regards to the corresponding class. However, the existing coverage criteria do
not take into account the output bias and compare the neurons outputs universally, making them less sensitive with the output impartiality. The existing work has demonstrated that some specific class could achieve very high coverage (\eg, neuron coverage)~\cite{ncmislead,nerualmisled}.



\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ4:}}
NPC and LNPC are strongly correlated with the output impartiality due to the construction of abstract CDPs for the prediction on each class. 
\end{tcolorbox}
\vspace{-.1in}
\section{Threats to Validity and Discussion}\label{sec:limit}
\paragraph{Threats to Validity}
First, the selection of the datasets and DNNs could be a threat to validity. In this work, we try to select the widely-used datasets and models in the recent works. 
Second, the configurable hyper-parameters could be a threat to validity such as $\alpha$, $\beta$, the number of clusters $k$ and the number of the buckets $m$. To counter this issue, we set different values of the parameters for the comparison.
Last, the generated datasets (\eg, RQ3 and RQ4) may be a threat. To mitigate the threat, we randomly select multple datasets and use the tool~\cite{ncmislead} with the same configuration to generate a large number of test suites for analysis. 

%widely used adversarial attack techniques to generate adversarial examples, and the tool~\cite{ncmislead} with the same configuration to generate a large number of test suites for correlation analysis. 


\paragraph{Limitation}
Like the coverage criteria in traditional software, we think there is no one best coverage criterion and each one has some limitations. The main advantage of NPC lies in its interpretability and the clear relationship with the internal decision of the DNN.
In this section, we summarize our limitation and discuss the potential solutions in the future.
\begin{itemize}
    \item Currently, our approach only considers the classification task instead of the regression tasks because the selected interpretation technique (\ie, LRP) does not support the DNN with regression prediction. The used interpretation technique is orthogonal with our approach and our approach is general as long as the critical neurons could be calculated.  We believe the interpretation techniques that work on regression tasks will further solve this problem.
    \item Our approach mainly works on feed-forward neural networks but not on recurrent neural networks (RNNs). This is because the number of iterations in the RNN is not fixed, which is a challenging for the interpretation (\eg, relevance calculation in LRP). In the future, we may extend LRP by unrolling the RNN to support RNN to solve this problem.
    %This work only demonstrates that NPC is correlated with defect detection and output impartiality, and we did not evaluate the correlation with other properties, such as naturalness~\cite{ncmislead} and robustness enhancement~\cite{dong2019limited}. Actually, it is an open question about whether the testing criteria should be correlated with such properties. We leave the evaluation as the future work.
\end{itemize}


% 1) regression
% 2) how to cluster
% 3) evluation metrics: naturalness, robustness
% 4) RNN

==> sections-old/evaluation.tex <==
\section{Evaluation}\label{sec:eval}

\revise{
\subsection{Setup}
To evaluate the effectiveness of our approach, we implemented the coverage criteria based on the PyTorch framework. 
This work is motivated by the recent findings ~\cite{ncmislead,nerualmisled,sekhon2019towards} on the limitation of the existing coverage criteria: \ding{172} the existing coverage criteria lack the interpretability and are unaware of the decision logic~\cite{nerualmisled,sekhon2019towards}, \ding{173} the existing coverage criteria are not sensitive to the defect detection including both of adversarial examples and natural errors~\cite{nerualmisled,ncmislead} and \ding{174} the existing coverage is not positively correlated with the output diversity~\cite{ncmislead}. Thus, we design the experiments to demonstrate the usefulness of our method in mitigating these challenges. Specifically, we aim to investigate and answer the following research questions:
}
% The objectives of the evaluation are to demonstrate that our approach is \textit{interpretable} and \textit{effective}. As we claimed in Section~\ref{sec:motivation}, a better coverage criterion should be interpretable, thus we first evaluate the usefulness of the CDP in interpreting the internal decision of the DNN (\textbf{RQ1} and \textbf{RQ2}). Motivated by the recent works~\cite{ncmislead,nerualmisled,dong2019limited}  that show the limitation of the existing coverage criteria, we then evaluate the effectiveness of NPC, \ie, whether there exists a correlation between defect detection and output impartiality (\textbf{RQ3} and \textbf{RQ4}).
% In particular, our experiments are designed to investigate and answer the following research questions:

\begin{itemize}[leftmargin=*]
     \item \textbf{RQ1}: How does the CDP affect the decision of the DNN? The CDP only selects the critical neurons in each layer. We design the experiment to evaluate whether such neurons are critical for DNN decisions.
    \item \textbf{RQ2}: How accurate is the abstract CDP in revealing internal decisions? Since the abstract CDP is extracted from CDPs of training samples in the corresponding cluster, we aim to evaluate whether the abstract CDP is still accurate in representing the DNN decision on these training samples in the cluster.
    \item \textbf{RQ3}: Is NPC sensitive with the errors including natural errors and adversarial examples? We investigate whether the proposed coverage criteria are sensitive in distinguishing the decision difference between erroneous samples and benign samples.
     \item \textbf{RQ4}: Is NPC correlated to the output impartiality? A test suite should exercise diverse behaviors and should not prefer only a few output values~\cite{nerualmisled}. We investigate whether the coverage criteria can reveal the impartiality of the test suite, \ie, the test suite with diverse behaviors should have high coverage while the test suite with biased behaviors should have low coverage.
    \item \textbf{RQ5}: How efficient is the calculation of NPC? Since NPC extracts decision behaviors based on the interpretation method, we investigate whether the interpretation analysis could introduce much time overhead for the coverage calculation. 
\end{itemize}


% \subsection{Research Questions}
% \begin{itemize}
%     \item \textbf{RQ1:}How accurate is the path extracted from the neurajl network?  
    
%     1) Single Image - Mask
%       path width: 1\%, 3\%, 5\%, 10\%
%       maks intervals: [0-1], [1-2],[2-3],[3-4]... [9-10],    10 
       
%       1\%
%     2) Mutiple images - Abstract Path - Mask - Effect
%       path width: 1\%   %, 3\%, 5\%, 10\%
%       maks intervals: [0-1], [1-2],[2-3],[3-4]... [9-10],    10 
%       cluster num: 1, 3, 5, 8 10
      
%      \item \textbf{RQ2:}
%      How useful the path in interpreting neural networks?
%      -- Cluster and Show images
%      1) visulize images in each cluster and calculate acc in each cluster.
%      2) the similarity in intra-class is less than inter-class?
%      intra-class in one cluster: average distance 
%      intra-class between two clusters: average distance
%      inter-class between two clusters: ...
     
     
%      3) the adversarial example vs original input?   0-1/4, 1/4-2/4, 2/4-3/4, 3/4-4/4, whole
%       4) Distinguish different adversarial attacks? original,  CW, FGSM, PGD  (1/4, 2/4, 3/4, 4/4)
%       original -> cw1, cw2, similarity 
     
%      c(2,4)
%      ori: cw
%      ori: pgd
%      ori: fgsm
%      cw: pgd
%      pgd1:Pgd2
    
      
     
%      \item \textbf{RQ3:}
%      Is the path coverage correlated to the defect detection?
     
%      -- prepare some test suites and calculate the correlation
%      \item \textbf{RQ4:}
%      Can the path coverage distinguish same-size test sets of natural examples with different levels of misclassification rates?
     
%      -- prepare some data included different number of natural errors
%      \item \textbf{RQ5:}
%      Is path coverage correlated to the output Impartiality?
     
%      --prepare some test suites and calculate the correlation
     
% \end{itemize}
\subsection{Subject Datasets and DNNs}
We selected three widely used datasets in the image classification domain and trained four models with competitive test accuracy, which are widely used in the previous works~\cite{ma2018deepgauge,test:surprise,pei2017deepxplore}.

\begin{itemize}[leftmargin=*]
    \item \textbf{MNIST}~\cite{mnist} is for handwritten digit image recognition (\ie, handwritten digits from $0$ to $9$), containing $60,000$ training data and $10,000$ test data. 
    %Each MNIST image is a single-channel of size $28 \times 28 \times 1$.
    We select the five layer Convolutional Neural Network~\cite{test:surprise} (named \emph{SADL-1}) and achieve an accuracy of 99.1\%.
    \item \textbf{CIFAR-10}~\cite{cifar} is a collection of images for general-purpose image classification, including $50,000$ training data and $10,000$ test data in $10$ different classes~(\eg, airplanes, cars, birds, and cats). 
    %Each CIFAR-10 image is three-channel of size $32 \times 32 \times 3$. 
    We select two models, \ie, the 12-layer Convolutional Neural Network~\cite{test:surprise} (named \emph{SADL-2}) and VGG16, which achieved the accuracy of 90.36\% and 89.17\%, respectively.
    \item \textbf{SVHN}~\cite{netzer2011reading} dataset is house numbers in Google Street View images, including 73,257 training data and 26,032 test data. We select the model AlexNet that has an accuracy of 94.31\%.
    \item \revise{\textbf{ImageNet} is a large-scale visual recognition challenge~(ILSVRC) dataset. The ImageNet contains a large number of training data~(\ie, over one million) and test data~(\ie, 50,000) with 1000 classes, each of which is of size $224 \times 224 \times 3$. To reduce the complexity of training and CDP evaluation, we select the first 10 classes to train a classifier with the model VGG16 that performs the classification on the 10 categories. The model is trained with an accuracy of 76.81\%.} 

% \noindent\textbf{ImageNet.} To further demonstrate that {\tool} scales to practical-sized dataset and DNN models, we also select ImageNet, which is a large-scale visual recognition challenge~(ILSVRC) dataset for general-purpose image classification. The complexity of ImageNet is characterized by a large number of training data~(\ie, over one million) and test data~(\ie, 50,000), as well as large data points, each of which is of size $224 \times 224 \times 3$ ($\sim 50$x dimensionality of CIFAR-10).
\end{itemize}
\subsection{Baselines}
We select the state-of-the-art coverage criteria as the baselines for the evaluation, \ie, Neuron Coverage (NC)~\cite{pei2017deepxplore}, $k$-Multisection Neuron Coverage (KMNC)~\cite{ma2018deepgauge}, Neuron Boundary Coverage (NBC)~\cite{ma2018deepgauge}, Likelihood-based Surprise Coverage (LSC)~\cite{ma2018deepgauge}, Distance-based Surprise Coverage (DSC)~\cite{test:surprise} and  Importance-Driven Coverage (IDC)\footnote{\color{red} Due to that the original IDC only supports Keras models, we implemented a PyTorch version of IDC for the comparison.}~\cite{IDCcov}.


% \begin{itemize}[leftmargin=*]
%     \item \textbf{Neuron Coverage (NC)}~\cite{pei2017deepxplore}, which measures the ratio of activated neurons of a DNN by a test suite. %We configure neuron coverage with different thresholds, \ie, 0.2, 0.5, 0.75.
%   \item \textbf{$k$-Multisection Neuron Coverage (KMNC)}~\cite{ma2018deepgauge}, which divides the the range of the neuron outputs (obtained from training data) into $k$ buckets. Then, KMNC measures the ratio of buckets of all neurons covered by a test suite.
%     % For a prediction, one section in each neuron will be covered. KMNC is a more fine-grained criterion that represents which sections of neurons are covered.
%     \item \textbf{Neuron Boundary Coverage (NBC)}~\cite{ma2018deepgauge}, which focuses on the corner-case buckets of the output of each neuron, and measures the ratio of corner-case buckets covered by a test suite. 
%     \item \textbf{Likelihood-based Surprise Coverage (LSC)}~\cite{test:surprise}, that measures the coverage based on the likelihood-based surprise, \ie, how diverse (surprise) is the test suite,
%     \item \textbf{Distance-based Surprise Coverage (DSC)}~\cite{test:surprise}, similarly, which measures the coverage based on the distance-based surprise.
% \end{itemize}
To be comprehensive, for NC, we set the threshold as 0, 0.2, 0.5 and 0.75 following~\cite{ncmislead}. For KMNC and NBC, we follow the configuration~\cite{ma2018deepgauge,test:deephunter} and set the $k$ value as 1,000 and 10. For LSC and DSC, we follow the configuration~\cite{test:surprise}, set the upper bound 2,000 and 2.0, respectively and set the number of buckets as 1,000. For the layer selection, we select the same layer in SADL-1 and SADL-2, which is used in~\cite{test:surprise}. For VGG16 in CIFAR and ImageNet, we select the last layer since it achieved the best result. For IDC, we follow the same configuration~\cite{IDCcov} and select the penultimate layer for each each model. In the selected layer, we choose the top 12 important neurons. For SNPC and ANPC, we set the number of buckets as 200 and the upper bound as 2.0. 

\subsection{RQ1: Relationship between CDP and the DNN Decision}

\begin{table*}[!t]
    \centering

    \scriptsize
    \caption{The average width (\%) and inconsistency rate (\%) after masking neurons in the CDP and NCDP}
    % Preview source code for paragraph 0
% Preview source code for paragraph 0

% Preview source code for paragraph 0
% Preview source code for paragraph 0

\begin{tabular}{cc|ccc|ccc|ccc|ccc}
\toprule 
 \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{$\alpha=0.7$} & \multicolumn{3}{c|}{$\alpha=0.8$} & \multicolumn{3}{c|}{$\alpha=0.9$} & \multicolumn{3}{c}{$\alpha=1$}\tabularnewline
% \cline{3-14}
 &  & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC & Width & Inc.C & Inc.NC\tabularnewline
\midrule 
\midrule 
MNIST & SADL-1 &  9.3 & 89.3 & 9.6 & \textbf{12.8} & \textbf{95.8} & \textbf{1.9} & 17.2 & 97& 0 & 33.3 & 98.9 & 1.8\tabularnewline
% \cline{2-14} \cline{3-14} \cline{4-14} \cline{5-14} \cline{6-14} \cline{7-14} \cline{8-14} \cline{9-14} \cline{10-14} \cline{11-14} \cline{12-14} \cline{13-14} \cline{14-14} 
\midrule
\multirow{2}{*}{CIFAR} & SADL-2 & \textbf{20.9} & \textbf{100} & \textbf{0} & 27.2 & 100 & 0 & 36.3 & 100 & 0 & 63.4 & 100 & 0\tabularnewline
 & VGG16 & 10.2 & 100 & 12.1 & {13.3} & {100} & {1.5} & \textbf{17.9}& \textbf{100} & \textbf{0.1} & 33.8 & 100 & 0\tabularnewline
% \cline{2-14} \cline{3-14} \cline{4-14} \cline{5-14} \cline{6-14} \cline{7-14} \cline{8-14} \cline{9-14} \cline{10-14} \cline{11-14} \cline{12-14} \cline{13-14} \cline{14-14} 
\midrule
SVHN & AlexNet & \textbf{23.0} & \textbf{100} & \textbf{2.1} & 29.6 & 100 &  1.2 & 38.2 & 100 & 0.2 & 64.6 & 100 & 0\tabularnewline
\midrule
\color{red}ImageNet &  \color{red}VGG16 &  \color{red}\textbf{41.1} &  \color{red}\textbf{99.3} &  \color{red}\textbf{12.5} &  \color{red}51.9 &  \color{red}99.8 &  \color{red} 13.9 &  \color{red}65.9 & \color{red}99.9 & \color{red}13.2 & \color{red}98.8 & \color{red}99.8 &\color{red}0.2
\tabularnewline
\bottomrule 
\end{tabular}

    \label{tab:singleinc}
\end{table*}
\subsubsection{Results of masking neurons of CDPs/NCDPs}
\paragraph{Mask all neurons.}
To evaluate whether the CDP has a critical impact on the decision of the DNN, we dropout outputs of neurons in the CDP (\ie, mask them as zero) and check whether the predicted result is inconsistent with the original result. Intuitively, we say that the CDP is accurate to reveal the decision if 1) the predicted output is largely affected after the neurons of the CDP are masked and 2) the predicted output is less affected after neurons in NCDP are masked. We extract CDPs for all training data and calculate the inconsistency rate after masking neurons in their CDPs and the corresponding NCDPs, respectively. 
\revise{
Specifically, the inconsistency rate of the classifier is defined as:
$$\frac{\{x |x\in X \wedge f(x)\neq f_m(x)\}}{|X|}$$
where $X$ is a set of test cases, $f(x)$ is the prediction result of the original classifier $f$ on the input $x$ and $f_m(x)$ is the prediction result after masking the CDP or NCDP of $x$. Intuitively, the higher the inconsistency rate, the larger the impact of the masked path.
}


Table~\ref{tab:singleinc} shows the average inconsistency rate by masking all neurons in the CDPs/NCDPs of all training data. The inconsistency rate shows the percentage of samples, whose prediction results are changed after the masking.  
To extract the path, we configure the parameter $\alpha$ (see Definition~\ref{def:cdp}) with different values, \ie, 0.7, 0.8, 0.9 and 1. Under each configuration, we show the average width of the CDP (Column \textit{Width}), which is the average ratio of neurons at each layer of the CDP, and the inconsistency rate after masking CDP (Column \textit{Inc.C}) and masking NCDP (Column \textit{Inc.NC}).


 The results show that the width of the CDP increases as the parameter $\alpha$ increases. For example, when $\alpha$ is 0.8, the average width on VGG-16 is 13.3\%, indicating that 13.3\% critical neurons are selected at each layer. When $\alpha$ is 1, the width becomes much larger (\ie, 33.8\%).
Furthermore, we found that almost all predicted results are changed when the CDPs are masked (\eg, for SADL-2 and VGG16, the inconsistency rate is 100\% for all configuration),
%for models in MNIST and CIFAR-10), 
which demonstrates that the CDP is very \textit{critical} for the decision. Conversely, when we mask other neurons that are not in the CDP (\ie, the NCDP), the inconsistency is very low (0\% to 3\%). In particular, when $\alpha$ is small, the width is small (\ie, less neurons are selected) and the performance is relatively low. For example, when $\alpha$ is 0.7, the inconsistency rate of masking CDP on SADL-1 is 89.3\%, which is lower than 98.9\% ($\alpha=1$);
The inconsistency rate of masking NCDP in CIFAR-VGG16 is much higher (12.1\%) than other configurations regarding $\alpha$, which shows that there are some critical neurons (in NCDP) that are missed. 
Based on the results in Table~\ref{tab:singleinc}, in the following experiments, we set $\alpha$ as 0.8, 0.7, 0.9, 0.7 and 0.7 for MNIST-SADL-1, CIFAR-SADL-2, CIFAR-VGG16 and SVHN-AlexNet and Imagenet-VGG16, respectively. We also evaluate the CDPs on test data and the results show the similar trends.



\revise{
\paragraph{Mask parts of neurons of CDPs.} To further evaluate the impact of CDP, we conduct a fine-grained evaluation that only masks a small part of neurons based on their relevance. Specifically, for a given CDP, we sort the neurons at each layer of the CDP and then split these sorted neurons into 5 equal buckets that have different relevance values, \ie, the top 20\% neurons with high relevance, the 20\%-40\% neurons, the 40\%-80\% neurons and the last 20\% neurons (\ie, 80\%-100\%) with low relevance. We get 5 sub-CDPs that contain neurons with different relevance values. Then we mask each of the sub-CDPs and calculate the inconsistency rate.
Table~\ref{tab:maskpart} shows the inconsistency rate by only masking parts of the CDP. Overall, we could find that the neurons with higher relevance can have larger impact on the prediction. After we mask the most important part (\ie, the top 20\% neurons), the largest inconsistency rate is caused, which indicates that these neurons have larger impact. When the last 20\% neurons are masked, the inconsistency rate is the smallest.

We also observe that the results depend on the tasks and models. For example, on CIFAR-VGG16, after masking the top 20\% neurons of CDPs, most inputs are inconsistent with the original prediction (97.94\%), which shows that these neurons are quite important for the prediction. However, for the model SADL-2, only 9.13\% inputs are inconsistent after masking the top 20\% neurons of the CDPs. Refer to the results in Table~\ref{tab:singleinc}, after masking all neurons in the CDP ($\alpha=0.7$), the inconsistency rate on SADL-2 becomes 100\%. It means that all neurons of the CDPs on SADL-2 are important for the prediction. 
Consider the results of CIFAR-VGG16 and ImageNet-VGG16, although the same model architecture is used, their results are not consistent, indicating that the CDPs are different on different datasets.
} 


%It is a trade-off between the width of the CDP and its representation on the decision logic. 




\begin{table}
\centering
\scriptsize
\caption{The average similarity of CDPs within a class or between different classes}
% Preview source code for paragraph 0

\begin{tabular}{cccccccccccccccc}
\toprule  
\multirow{2}{*}{$\alpha$} & \multicolumn{3}{c}{SADL-1} & \multicolumn{3}{c}{SADL-2} & \multicolumn{3}{c}{VGG16(CIFAR-10)} & \multicolumn{3}{c}{AlexNet} & \multicolumn{3}{c}{\color{red}VGG16(ImageNet)}\tabularnewline
\cline{2-16} \cline{3-16} \cline{4-16} \cline{5-16} \cline{6-16} \cline{7-16} \cline{8-16} \cline{9-16} \cline{10-16} \cline{11-16} \cline{12-16} \cline{13-16} 
 & Width & Intra & Inter & Width & Intra & Inter & Width & Intra & Inter & Width & Intra & Inter & \color{red}Width & \color{red}Intra & \color{red}Inter\tabularnewline
\midrule
\midrule
0.7 & 9.30\% & 57.7\% & 34.7\% & 20.9\% & 48.6\% & 23.2\% & 10.2\% & 86.5\% & 22.2\% & 23.0\% & 47.8\% & 30.0\%& \color{red}41.1\%& \color{red}54.9\%& \color{red}32.2\%\tabularnewline
0.8 & 12.80\% & 62.8\% & 39.1\% & 27.2\% & 56.5\% & 41.8\% & 13.3\% & 60.9\% & 26.0\% & 29.6\% & 54.5\% & 36.5\% & \color{red}51.9\% &\color{red} 60.8\% & \color{red}41.6\%\tabularnewline
0.9 & 17.20\% & 67.6\% & 45.3\% & 36.3\% & 64.4\% & 38.0\% & 17.9\% & 67.1\% & 32.0\% & 38.2\% & 63.2\% & 46.1\% & \color{red}65.9\% & \color{red}70.9\% & \color{red}55.8\%\tabularnewline
1 & 33.30\% & 74.5\% & 56.3\% & 63.4\% & 86.5\% & 62.0\% & 33.8\% & 78.3\% & 56.1\% & 64.6\% & 78.3\% & 75.4\%& \color{red}98.8\%& \color{red}99.9\%& \color{red}97.9\%\tabularnewline
\bottomrule 
\end{tabular}

% \begin{tabular}{cccccc}
% \hline 
%  &  & $\alpha=0.7$ & $\alpha=0.8$ & $\alpha=0.9$&$\alpha=1$\tabularnewline
% \hline 
% \multirow{3}{*}{SADL-1} & Width & 9.30\% & 12.80\% & 17.20\% & 33.30\%\tabularnewline
%  & Intra-Class & 57.70\% & 62.80\% & 67.60\% & 74.50\%\tabularnewline
%  & Inter-Class  & 34.70\% & 39.10\% & 45.30\% & 56.30\%\tabularnewline
% \hline 
% \hline 
% \multirow{3}{*}{SADL-2} & Width & 20.90\% & 27.20\% & 36.30\% & 63.40\%\tabularnewline
%  & Intra-Class & 48.60\% & 56.50\% & 64.40\% & 86.50\%\tabularnewline
%  & Inter-Class & 23.20\% & 41.80\% & 38.00\% & 62.00\%\tabularnewline
% \hline 
% \hline 
% \multirow{3}{*}{VGG16} & Width & 10.20\% & 13.30\% & 17.90\% & 33.80\%\tabularnewline
%  & Intra-Class & 86.50\% & 60.90\% & 67.10\% & 78.30\%\tabularnewline
%  & Inter-Class & 22.20\% & 26.00\% & 32.00\% & 56.10\%\tabularnewline
% \hline 
% \hline 
% \multirow{3}{*}{AlexNet} & Width & 23.00\% & 29.60\% & 38.20\% & 64.60\%\tabularnewline
%  & Intra-Class & 47.80\% & 54.50\% & 63.20\% & 78.30\%\tabularnewline
%  & Inter-Class & 30.00\% & 36.50\% & 46.10\% & 75.40\%\tabularnewline
% \hline 
% \end{tabular}
% \begin{tabular}{ccccc}
% \toprule
%  & $\alpha=0.7$ & $\alpha=0.8$ & $\alpha=0.9$ & $\alpha=1$\tabularnewline
% \midrule 
% \midrule
% Width & 9.3\% & 12.8\% & 17.2\% & 33.3\%\tabularnewline
% \midrule 
% Intra-Class & 0.347 & 0.391 & 0.453 & 0.563\tabularnewline
% Inter-Class & 0.577 & 0.625 & 0.676 & 0.745\tabularnewline
% \bottomrule
% \end{tabular}
\label{tab:distance}
\end{table}


\begin{table}[]
    \centering
   \small
    \caption{The average inconsistency rate (\%) after masking parts of neurons in the CDP.}
  \color{red}{  \begin{tabular}{cc|ccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{5}{c}{Inconsistency Rate}\tabularnewline
\cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 &  & 20\% & 20\%-40\% & 40\%-60\% & 60\%-80\% & 80\%-100\%\tabularnewline
 \midrule
 \midrule
MNIST & SADL-1 & 99.13 & 97.53 & 92.46 & 79.73 & 49.02\tabularnewline
 \midrule
\multirow{2}{*}{CIFAR} & SADL-2 & 9.13 & 7.65 & 3.29 & 2.39 & 0.58\tabularnewline
 & VGG16 & 97.94 & 84.13 & 62.42 & 43.21 & 22.64\tabularnewline
SVHN & AlexNet & 99.96 & 99.45 & 78.7 & 42.86 & 15.95\tabularnewline
 \midrule
ImageNet & VGG16 & 73.22 & 27.02 & 15.07 & 9.91 & 6.21\tabularnewline
\bottomrule
\end{tabular}
}
    \label{tab:maskpart}
\end{table}

\subsubsection{Results on effect of the width.}
% \paragraph{Setup} 

The width of the CDP may affect its accuracy
in representing the decision logic. If the width is too large, the CDP contains some non-critical neurons that may also be included in other CDP, making it hard to distinguish them. \revise{We investigate the similarity between different classes. Specifically, for each class, we randomly select 100 test data that is correctly predicted as the target class. Then we calculate the average similarity of CDPs in the same class or between different classes as follows:
$$Intra=avg(\{sim(x^y_i, x^y_j) | y\in Y \wedge i\neq j \wedge x^y_i\in X^y \wedge x^y_j\in X^y\}) $$
$$Inter=avg(\{sim(x^{y_m}_i, x^{y_n}_j) | y_m\in Y \wedge y_n\in Y \wedge m\neq n \wedge x^{y_m}_i\in X^{y_m} \wedge x^{y_n}_j\in X^{y_n}\}) $$
where $Y$ is the set of all classes, $X^y$ is a set of test data (its size is 100) in the class $y$, $sim(x, y) = \frac{\sum_{l\in f}J_{p^l_x,p^l_y}}{|f|}$ represents the similarity between CDPs of $x$ and $y$ (see Equation~\ref{sec:jaccard}). Intuitively, the similarity between CDPs of the same class should be greater than the similarity between CDPs of two different classes.
}

Table~\ref{tab:distance} shows the average similarity between two CDPs in the same class (\ie, Column \textit{Intra}) and in different classes (\ie, Column \textit{Inter}) on the training data. The results show that the average similarity increases with the increase of the width, which further demonstrates that, if the CDP is too wide, it is not accurate to show the decision difference on two inputs. If the width of the CDP is too small, then it may miss some critical neurons (see Table~\ref{tab:singleinc}).

%or too small, the CDP may include more non-critical neurons or miss more critical neurons, making it hard to distinguish the logic of two inputs well. Fig.~\ref{XXX}...
%Our goal is to select the CDP, which has smaller width (\ie, the CDP is representative) and could can represent the decision logic accurately, \ie, the CDP is important for decision-making and the corresponding NCDP is not important for decision-making. 


%\textbf{Performance.} The average time spent for extracting the CDP of an input is \fei{}, \fei{}, \fei{} and \fei{}, respectively. 


\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ1:}} 
CDPs are critical for the prediction while NCDPs are not critical, which reveals that the CDPs are more relevant to the internal decision logic of the DNN.
%\fei{In addition, the width of the CDP is sensitive for representing the decision of the DNN.}
%With path abstraction, we could reduce the total number of CDPs. The abstract CDP could become narrow (\ie, smaller width) while the performance is still competitive. 
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}

%$\alpha=0.9$ because it could achieve similar accuracy with $\alpha=1$, but the width of CDPs is much smaller.
%and the inconsistency rate of masking NCDP in VGG16 (22\%) is much higher than other two configurations.




% Specifically, we evaluate the accuracy of the 
% single CDP and the abstract CDP. For the single CDP, we extract CDPs for 10,000 test data in each dataset, and calculate the inconsistency rate, \ie, how many test data whose result will be inconsistent by masking neurons in their CDPs and the corresponding NCDPs, respectively. 

%For abstract CDPs in the decision graph, some training samples (in the cluster of a class) share the same abstract CDP, we mask the neurons of this abstract CDP and check the inconsistency rate of all training samples in this cluster. Finally, we calculate the average inconsistency rate of all clusters in different classes.

%\paragraph{Accuracy of Single CDPs}

\subsection{RQ2: Effectiveness of Path Abstraction}
\paragraph{Setup.} Since the abstract path represents the decision logic of training samples in the corresponding cluster, we first investigate whether the abstract path is still critical for the prediction of inputs in the cluster. Similar to RQ1, we mask the abstract CDP/NCDP and see the average inconsistency rate of training inputs in the cluster. Then, we evaluate whether the path abstraction could identify similar decision logic by measuring the similarity with or without clustering. 
\revise{ Specifically, for each cluster that contains a set of training samples $X$, we can calculate its abstract CDP based on all CDPs of $X$. To evaluate the precision of the path abstraction, for every input $x\in X$, we masked the same neurons (\ie, the abstract CDP) and evaluate the average inconsistency rate. Note that, in RQ1, we mask different neurons for different inputs of $X$ based on their individual CDPs while we mask the same neurons (in the abstract CDP) for all inputs of $X$ in RQ2. %We could compare the results of RQ1 and RQ2 to see the precision of the abstraction.
}

\subsubsection{Impact on prediction}
For the path abstraction of each DNN, we investigate a total of 16 configurations with different parameters $(k, \beta)$, where $k$ is the number of the clusters in each class and $\beta$ is the threshold to select neurons with high weights (the first column in Table~\ref{tab:abstractp}). Note that, when $k=1$, the abstract CDP is extracted by merging CDPs of all inputs that are predicted as the same class.

The results in Table~\ref{tab:abstractp} show that, with the increase of the number of clusters, the width tends to be slightly larger in most cases under the same threshold $\beta$ (see Column \textit{Wid.}), indicating that the average weight of neurons is also larger (\ie, CDPs in each cluster share more common neurons).
\revise{We count the number of the change of Inc.C and found that 81.25\% (39/48) of the Inc.C change is increasing or unchanged when the number of clusters increases. More fine-grained clustering (\ie, more clusters) could merge the similar CDPs together, by which the abstract CDP is more \textit{stable} (larger average weights) and \textit{accurate} (higher inconsistency rate after masking CDPs).
The results demonstrate the usefulness of clustering and merging.}
%
%(see Column \textit{Inc.C}/Column \textit{Inc.NC}). 

% or decreasing between the change of the parameter $k$. For example, when $\beta=0.6$, 




\begin{table}[!t]
    \centering
    \scriptsize
    % Preview source code for paragraph 0

    \caption{The average width and inconsistency rate (\%) after masking neurons in the abstract CDP and NCDP}
    % Preview source code for paragraph 0
% Preview source code for paragraph 0

\begin{tabular}{ccccccccccccccccccc}
\toprule
\multirow{2}{*}{($k$, $\beta$)} & \multicolumn{3}{c}{SADL-1} & \multicolumn{3}{c}{SADL-2} & \multicolumn{3}{c}{VGG16(CIFAR-10)} & \multicolumn{3}{c}{AlexNet} & \multicolumn{3}{c}{\color{red}VGG16(ImageNet)}\tabularnewline
\cline{2-13} \cline{3-13} \cline{4-13} \cline{5-13} \cline{6-13} \cline{7-13} \cline{8-13} \cline{9-13} \cline{10-13} \cline{11-16} \cline{12-16} \cline{13-16} 
 & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & \color{red}Wid. & \color{red}Inc.C & \color{red}Inc.NC\tabularnewline
\midrule 
\midrule 
(1, 0.6) & 16.9 & 93.6 & 2.3 & 13.9 & 99.9 & 2.4 & 15.5 & 99.8 & 4.3 & 17.3 & 99.4 & 4.9 & \color{red}41.5	& \color{red}99.8	& \color{red}1.7\tabularnewline
(1, 0.7) & 14.6 & 89.2 & 8.4 & 9.4 & 99.8 & 2.4 & 13.1 & 99.3 & 4.3 & 13.6 & 99.1 & 13.9 & \color{red}34.4 &\color{red} 99.8 & \color{red}1.7\tabularnewline
(1, 0.8) & 12.5 & 78.8 & 29.9 & 6.4 & 99.2 & 2.4 & 10.8 & 98.8 & 4.3 & 9.8 & 96.3 & 16.3& \color{red}26.4 & \color{red}99.8 & \color{red}1.7\tabularnewline
(1, 0.9) & 10.4 & 73.6 & 59.8 & 4.1 & 90.9 & 2.4 & 7.9 & 100 & 10.1 & 5.7 & 50.9 & 37.6 & \color{red}17.7 & \color{red}99.8 &\color{red}1.7\tabularnewline
\midrule 
\midrule 
(4, 0.6) & 16.7 & 94.5 & 2.4 & 14.6 & 99.9 & 2.0 & 15.8 & 99.9 & 4.3 & \textbf{18.5} & \textbf{99.5} & \textbf{4.4}&\color{red}54.5&\color{red}100&\color{red}2.9\tabularnewline
(4, 0.7) & 15.4 & 95 & 2.5 & 10.8 & 99.9 & 2.0 & 13.5 & 99.9 & 4.8 & 15.1 & 99 & 5.8&\color{red}\textbf{49}&\color{red}\textbf{100}&\color{red}\textbf{1.9}\tabularnewline
(4, 0.8) & \textbf{14.6} & \textbf{94.1} & \textbf{3.9} & 7.6 & 99.6 & 2.0 & 11.2 & 99.9 & 4.8 & 11.8 & 96.4 & 16.2& \color{red}40.4&	\color{red}100	&\color{red}2.67\tabularnewline
(4, 0.9) & 12.2 & 88.1 & 14.3 & 4.8 & 95.3 & 2.0 & 8.4 & 100 & 9.2 & 7.6 & 80 & 26.7&\color{red}34.3	&\color{red}100&\color{red}2.6\tabularnewline
\midrule 
\midrule 
(7, 0.6) & 16.9 & 96.3 & 2.6 & 14.9 & 99.9 & 1.5 & 15.9 & 99.8 & 2.8 & 18.4 & 99.4 & 5.6&\color{red}64.2&\color{red}100&\color{red}4.3\tabularnewline
(7, 0.7) & 15.9 & 96.1 & 3.2 & 11.2 & 99.8 & 1.5 & 13.7 & 99.9 & 3.5 & 15.2 & 98.9 & 6&\color{red}59.5&\color{red}100&\color{red}2.9\tabularnewline
(7, 0.8) & 14.6 & 92.5 & 2.9 & 7.9 & 99.7 & 1.5 & 11.4 & 99.9 & 4.4 & 12.1 & 97.6 & 9.7& \color{red}51.8& \color{red}100& \color{red}3.6\tabularnewline
(7, 0.9) & 12.5 & 88.7 & 9.5 & \textbf{5.4} & \textbf{98.2} & \textbf{1.6} & \textbf{8.7} & \textbf{100} & \textbf{4.9} & 8 & 90.5 & 19&\color{red}46.7&\color{red}100	&\color{red}3.1\tabularnewline
\midrule 
\midrule 
(10, 0.6) & 16.9 & 95.3 & 1.7 & 15.2 & 99.9 & 1.1 & 15.9 & 99.9 & 2.0 & 18.5 & 99.4 & 5.2&\color{red}73.2&\color{red}100&\color{red}4.3\tabularnewline
(10, 0.7) & 16.1 & 95.1 & 3.1 & 11.5 & 99.8 & 1.2 & 13.7 & 99.9 & 2.7 & 15.4 & 98.9 & 6.3&\color{red}70.5&\color{red}100&\color{red}4.3\tabularnewline
(10, 0.8) & 14.6 & 93.0 & 4.3 & 8.3 & 99.8 & 1.3 & 11.5 & 99.9 & 3.4 & 12.4 & 98.4 & 8.5&\color{red}58.3&\color{red}100&\color{red}3.9\tabularnewline
(10, 0.9) & 13.5 & 89.2 & 8.8 & 5.4 & 98.8 & 1.3 & 8.7 & 99.9 & 8.8 & 8.6 & 92.9 & 17.7&\color{red}54.3&\color{red}100&\color{red}2.7\tabularnewline
\bottomrule 
\end{tabular}


% % Preview source code for paragraph 0

% \begin{tabular}{c|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{\#Cluster} & \multicolumn{3}{c|}{SADL-1 ($\beta=0.8$)} & \multicolumn{3}{c|}{SADL-2 ($\beta=0.9$)} & \multicolumn{3}{c|}{VGG16 ($\beta=0.9$)} & \multicolumn{3}{c}{AlexNet ($\beta=0.6$)}\tabularnewline
% % \cline{2-13} 
%  & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC & Wid. & Inc.C & Inc.NC\tabularnewline
% \midrule
% \midrule 
% 1 & 12.5 & 78.8 & 29.9 & 4.1&	90.9 &	2.4
% %3.3 & 82.1 & 9.7 
% & 7.9 & 100 & 10.1 &17.3  & 99.4  &4.9 \tabularnewline
% 4 & \textbf{14.6} & \textbf{94.1} &\textbf{ 3.9 }&
% %5.1 & 94.3 & 5.6 
% 4.8	& 95.3	& 2 & 8.4 & 100 & 9.2 & 
% \textbf{18.5} & \textbf{99.5 }& \textbf{4.4} \tabularnewline
% 7 & 14.6 & 92.5 & 2.9 & 
% %5.9 & \textbf{98.7 }& \textbf{0} 
% \textbf{5.4}	& \textbf{98.2}&\textbf{	1.6}& \textbf{8.7} & \textbf{100 }& \textbf{4.9} & 
% 18.4 &99.4  &5.6 \tabularnewline
% \bottomrule 
% \end{tabular}


    \label{tab:abstractp}
\end{table}

Compared with the results on single CDPs (Table~\ref{tab:singleinc}), we found that the abstract path could still achieve competitive performance and even better than single CDPs on some models. 
 It means that the path abstraction can be used to select commonly important neurons for all training data in a specific cluster (\ie, high inconsistency rate after masking CDPs and low inconsistency rate after masking NCDPs).
For example, on SADL-2, the inconsistency rates of CDP and NCDP are 98.2\% and 1.6\% ($k=7$), which are close to results of single CDPs (\ie, 100\% and 0\%) and the width is much smaller (\eg, 5.4\% for abstract CDPs and 27.2\% for single CDPs). For AlexNet, using the abstraction in the cluster, we could select more accurate CDPs (\eg, the average width of the abstract CDPs and the single CDPs is 18.5\% and 23.0\%).
Finally, in the following experiments, we select the configuration (4, 0.8), (7, 0.9), (7, 0.9), (4, 0.6) and (4, 0.7) as the parameters for SADL-1, SADL-2, VGG-16, AlexNet and VGG-16 (ImangeNet), respectively (the bold numbers).
%Based on the results in Table~\ref{sec:pathabstract}, 
%For VGG16, when $k=7$, the results are better than results of single CDPs with $\alpha=0.8$. Specifically, the abstract CDPs are more accurate, \ie, they have the same  inconsistency rate on CDPs (100\%) but smaller on NCDPs (4.9\% and 22.4\%). 
%Moreover, based on the statistical analysis in the cluster, path abstraction could help further reduce the width of the abstract CDPs. For example, for the SADL-2, we could  is 
%abstract CDPs with small width and high accuracy.

\subsubsection{Decision Revealing}
% Preview source code for paragraph 0
Table~\ref{tab:clustersim} shows the results on the average similarity with and without clustering. Column \textit{\#Clus.} shows the number of clusters configured for each model. Without clustering, Column \textit{\#Intra\_Cla.} shows the average similarity between CDPs that are in the same class (\ie, the intra-class similarity). Column \textit{\#Inter\_Cla.} shows the average similarity between CDPs that belong to different classes (\ie, the inter-class similarity). After the clustering, we show the average similarity between CDPs in the same cluster (\ie, intra-cluster similarity shown in Column \textit{\#Intra\_Clus.}) and the average similarity between CDPs in different clusters of the \emph{same} class (\ie, inter-cluster similarity shown in Column \textit{\#Inter\_Clus.}). Note that inter-cluster similarity only compares clusters that belong to the same class

Comparing the results between intra-class similarity (without clustering) and intra-cluster similarity (with clustering), we found that the average similarity increases (\eg, from 0.625 to 0.708 in SADL-1). In particular, in the same class, the inter-cluster similarity is much smaller than intra-cluster similarity although the two clusters belong to the same class (\eg, 0.708 for intra-cluster and 0.381 for inter-cluster).
Moreover, the inter-cluster similarity is even close to the inter-class similarity. The results show that samples in the same class could have different decision logic (\eg, the black dogs and white dogs may be different). By the path abstraction, we generate fine-grained CDPs which could distinguish such differences well.

Fig.~\ref{fig:clustervis} shows some examples whose CDPs are clustered into different groups (on SADL-1). Each row represents one cluster.
We can observe that, from the human's perception, the inputs in the same cluster look very similar. For example, the digit ``4'' looks similar to the digit ``9'' in the fourth cluster and the digit ``5'' has a slight deflection in the first cluster. The results further show that inputs that trigger the similar decision logic is likely to be grouped into one cluster based on the extracted CDPs.

\begin{table}[!t]
    \centering
    \small
    \caption{The average similarity with and without clustering}
\begin{tabular}{cccccc}
\toprule 
Model & \#Clus. & Intra\_Cla. & Inter\_Cla. & Intra\_Clus. & Inter\_Clus.\tabularnewline
\midrule 
\midrule 
SADL-1 & 4 & 0.628 & 0.391 & 0.708 & 0.381\tabularnewline
SADL-2 & 7 & 0.486 & 0.232 & 0.524 & 0.260\tabularnewline
VGG16(CIFAR-10) & 7 & 0.671 & 0.320 & 0.703 & 0.316\tabularnewline
AlexNet & 4 & 0.478 & 0.300 & 0.524& 0.298 \tabularnewline
\color{red}VGG16(ImageNet) &\color{red}4	&\color{red}0.549&	\color{red}0.322&	\color{red}0.546&	\color{red}0.331\tabularnewline
\bottomrule 
\end{tabular}
    \label{tab:clustersim}
\end{table}
\begin{figure}
    \centering
     \includegraphics[width=0.90\linewidth]{pics/show_case.pdf}
    \caption{Inputs sampled from clusters in the class 4 and 5}
    \label{fig:clustervis}
\end{figure}


\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ2:}} 
\revise{Based on the aggregation (\ie, union) of all CDPs in each cluster}, the abstract CDP is still critical for predicting inputs in a cluster. Moreover, the abstract CDP is sensitive to reveal different decision logic. Inputs in the same cluster have similar decision and inputs in different clusters of the same class tend to have different decision behavior.
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}
\vspace{-.1in}
\subsection{RQ3: Sensitivity with Defect Detection}
\paragraph{Setup.} 
Motivated by~\cite{ncmislead,nerualmisled}, this experiment evaluates the effectiveness in detecting defects including the natural errors and the adversarial examples. We follow the similar design in~\cite{nerualmisled}: first, we randomly select 1,000 benign samples (denoted as $s_0$) from the test data. 
Then, we construct several test suites by replacing a small number of samples of $s_0$ with the same number of errors such that they have the same size.
To be specific, for natural errors, we select a certain number of inputs from test data in each class, which are predicted incorrectly. For adversarial examples, we adopt the PGD attack~\cite{madry2018towards} to generate a large number of adversarial examples, some of which are then randomly selected in each class. For natural errors and adversarial examples, we generate 6 test suites including different numbers of errors (\ie, 1\%, 2\%, 3\%, 5\%, 7\%, 10\%), respectively. We use $S$ to denote the set of the test suites including the initial set $s_0$.
\revise{To reduce the randomness, we repeat the process 5 times and calculate the average results.}
%The expectation is that the code coverage should be sensitive in different numbers of errors.

\paragraph{Results.} Fig.~\ref{fig:coveragechange} shows the results on the test suites including a different number of errors. 
To conduct the comparison between different approaches, all the coverage is normalized to [-1,1]. \revise{Specifically, for each test suite $s\in S$, we calculate its coverage change compared with the initial test suite $s_0$ with regard to the coverage criterion $Cov$, \ie,  $\Delta = \{Cov(s)-Cov(s_0)|  s\in S \}$.
For each $s\in S$, we normalize the change of the coverage as follows:

\begin{equation}
\label{equa:mutation}
NCov(s) = \frac{Cov(s)-Cov(s_0)}{max(\Delta)-min(\Delta)}
\end{equation}
Note that the coverage change can be negative value.
%where $min=min$ and $max$ are the minimum coverage change and the maximum coverage change for all test suites $S$, respectively. 

} 



The first row shows the average results on natural errors (\emph{Nat.}) and the second row shows the results on adversarial examples (\emph{AE}). The horizontal axis represents the percentage of errors while the vertical axis represents the normalized coverage.

The results show that the coverage criteria exhibit different performance on different number of errors. \revise{In general, we could find that SNPC and ANPC tend to be more stable than other methods in terms of the sensitivity to errors.  In most cases, the trends of SNPC and ANPC are in line with the expectations, \ie, the coverage can increase when more errors (adversarial examples or natural errors) are introduced. NBC is the most unstable one because it mainly focuses on the boundary behaviors of the model. For KMNC and NC (with threshold 0.5), we observe that they perform better in natural errors than adversarial examples. The coverage of NC and KMNC increases when the number of natural errors increase. However, their coverage does not always increase on adversarial examples. Particularly, KMNC decreases on AEs of CIFAR-VGG16, ALexNet and ImageNet-VGG16. We conjecture that KMNC mainly considers the major functionality of the DNN while ignores the boundary functionality, thus replacing some benign samples with the corner cases (\eg, adversarial examples) could decrease the diversity of major behavior. LSC performs better in most cases but is insensitive in AlexNet, \ie, the coverage does not change on both adversarial examples and natural error of AlexNet, which indicates that 
the DNN may have a large impact on LSC. DSC is not sensitive on natural errors while it is better on adversarial examples. It is worth pointing out that most coverage criteria tend to have irregular change in AE (AlexNet) while SNPC still has an increasing trend.

Considering IDC that is also based on LRP, we can observe that the coverage increase is not as stable as SNPC and ANPC, \eg, on Nat.(AlexNet), AE (SADL-2), AE (AlexNet) and AE (IVGG). Although both IDC and NPC adopt LRP, NPC is more fine-grained than IDC. IDC only considers one layer and the fixed critical neurons in this layer, which is coarse. Differently, NPC considers critical neurons along different layers (\ie, CDP), and the fine-grained CDP-based clustering is performed in each class. Thus, our results tend to be more stable.


Moreover, we also observe that there are some correlations between these coverage. Specifically, the trend of coverage increase with regards different coverage criteria could be similar. For example, in Nat.(SDAL-1), LSC, DSC, ANPC and SNPC have the similar trend. In Nat.(SADL-2), SNPC and NC have the similar trend. Most of the coverage criteria have the similar trend in Nat.(VGG16), Nat.(IVGG) and AE(SADL-1). 
}


% For example, consider the natural errors at the first row, SNPC and DSC achieve the best results, \ie, the coverage increases when the number of nature errors increases, indicating such two coverage criteria are more sensitive to nature errors. ANPC performs better on SADL-1 and VGG-16, but not well on SADL-2 and AlexNet. We made an in-depth analysis and found that the introduced nature errors have similar activation values along the abstract path, making ANPC hard to distinguish them.  For others, NC with all four thresholds (denoted as NC-ALL) does not change much (\ie, $y$=0), indicating that NC is too coarse-grained. KMNC shows a decreasing trend, which seems to be aligned in its design, \ie, they mainly cover the major function of DNNs. Hence, when some benign samples are replaced with errors that may cover corner cases, the coverage of the major region decreases. 
% LSC increases on SADL-1 and VGG-16 but does not change on SADL-2 and AlexNet.

% but it is not accurate in SADL-1 (\eg, the coverage does not change after adding 5\% and 10\% errors).
% Note that, LSC does not change on SADL-2 because the Surprise Adequacy value is NaN and Inf in almost all layers. Compared with LSC and DSC, our method considers the relationship between all layers and does not rely on the selection of layers. 


% as the number of natural errors increases, NPC and LNPC increase in all three models. It is because new decision logic is triggered by the natural errors and our method is sensitive in such new decision behavior. Similarly, DSC also increases during the increase of errors.


%However, the existing structural coverage criteria are not sensitive in the new errors. 


%LSC and DS shows a certain degree of increasing trend on SADL-1 and VGG16 but does not change on SADL-2. 

% Consider adversarial examples in the second row, we observed that ANPC achieves the best result, \ie, it always increases in four models when the number of adversarial examples increases. However, SNPC performs worse on AEs than nature errors. Our in-depth analysis shows that the PGD attack adopts the gradient-based strategy that tends to generate inputs towards one direction, making the adversarial example close to the prediction of the specific class. Finally, the paths of AEs and benign samples (in the same class) are similar, but the activation values are very different. For example, after the attack, a dog may be predicted as the cat, however, the predicted confidence is usually low (\eg, less than 80\%), which makes the data-flow sensitive coverage (\ie, ANPC) distinguish AEs well. Consider other coverage criteria, we found that the results are not stable among different models. For example, all coverage criteria perform well on SADL-1. KMNC performs well on SADL-2 but not well on VGG-16 and AlexNet. DSC works well on VGG-16 but not well on SADL-2 and AlexNet.

%From the results of natural errors and adversarial examples, we could observe that SNPC performs better in detecting natural errors while ANPC performs better in detecting adversarial examples. 

% From the results of natural errors and adversarial examples, we could conclude that natural errors introduce more information (\ie, trigger more different decision) than the adversarial examples.

% the coverage usually decreases as the number of the adversarial examples increases. On SADL-2 and VGG16, we could still observe the similar trend with existing coverage criteria (\eg, the coverage increases firstly and then decreases). Surprisingly, on ASDL-1, we achieved totally different results, \ie, the coverage decreases as the adversarial examples are adding.   
% We made a deep analysis and found the following two possible reasons, 1) although the number of adversarial examples increases, many of them are more close to the corresponding abstract CDP than the natural samples (\ie, triggered the known logic). It is because the PGD attack adopts the gradient-based that tends to generate inputs towards one direction, making the adversarial example close to the prediction of the specific class. 2) many adversarial examples are predicted into one specific class (\ie, the prediction is biased to one class), which decreases the output impartiality (see the Results in RQ4). Thus the coverage is slightly decreased.
%trigger similar decision logic. Meanwhile, we removed the same number of benign samples, which actually trigger more diverse decision than the inserted adversarial samples.  

%However, we could still found that there are some similar trend between our coverage and the existing criteria. For example, on SADL-2, similar with KMNC and NBC, the coverage of NPC and LNPC 
%is decreased to the minimum when 20\% adversarial examples are introduced. On VGG16, similar with KMNC, NBC and LSC, the coverage of LNPC increases when the number of adversarial examples increase by 1\%, 3\%, 5\%, 10\% and 15\% but decrease after 20\% adversarial examples are introduced in the test suite.


\begin{figure}
    \centering
    % \includegraphics[width=1\linewidth]{pics/defecttrend.pdf}
     \includegraphics[width=1.1\linewidth]{imgs/error_avg.pdf}
    \caption{Coverage change on test suits including different number of errors.}
    \label{fig:coveragechange}
\end{figure}

% Preview source code for paragraph 0
\begin{table*}[]
    \centering
    % \scriptsize
    \caption{Correlation between coverage criteria and output impartiality}
    % Preview source code for paragraph 0
\scriptsize
\begin{tabular}{ccccccccccccc}
\toprule 
 &  & KMNC & NBC & NC(0.0) & NC(0.2) & NC(0.5) & NC(0.75) & LSA & DSA &\color{red} IDC& ANPC & SNPC\tabularnewline
\midrule 
\midrule 
\multirow{5}{*}{size=100} & SADL-1 & -0.262 & -0.262 & -0.300 & 0.099 & 0.315 & 0.001 & 0.000 & -0.638 & \color{red}-0.360& {-0.244} & \textbf{0.723}\tabularnewline
 & SADL-2 & -0.029 & -0.029 & \textbf{0.553} & -0.397 & -0.065 & -0.111 & 0.000 & 0.181 &\color{red} \textbf{0.587} & \textbf{0.482} & \textbf{0.789}\tabularnewline
 & VGG16 & -0.348 & -0.348 & 0.037 & -0.031 & -0.210 & -0.273 & 0.000 & -0.145 & \color{red} 0.052& 0.012 & -0.055\tabularnewline
 & AlexNet & -0.457 & \textbf{0.593} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -0.320 & \color{red} \textbf{0.912} & \textbf{0.961} & \textbf{0.989}\tabularnewline
 \cline{2-13}
 & Avg. & -0.274 & -0.011 & 0.072 & -0.082 & 0.010 & -0.096 & 0.000 & -0.230 &\color{red} \textbf{0.298 } & \textbf{0.601} & \textbf{0.612}\tabularnewline
\midrule 
\midrule 
\multirow{5}{*}{size=500} & SADL-1 & \textbf{0.639} & -0.116 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -0.639 & \color{red} -0.707& \textbf{0.340} & \textbf{0.870}\tabularnewline
 & SADL-2 & \textbf{0.543} & 0.041 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.330 &\color{red} \textbf{0.473} & \textbf{0.584} & \textbf{0.817}\tabularnewline
 & VGG16 & \textbf{0.414} & \textbf{0.589} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -0.255 &\color{red} \textbf{ 0.210}& \textbf{0.141} & \textbf{0.821}\tabularnewline
 & AlexNet & \textbf{0.539} & \textbf{0.586} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -0.170 & \color{red}\textbf{0.931}&\textbf{0.908} & \textbf{0.974}\tabularnewline
  \cline{2-13}
 & Avg. & \textbf{0.534} & 0.275 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -0.184 & \color{red} \textbf{0.227} & \textbf{0.893} & \textbf{0.871}\tabularnewline
\bottomrule 
\end{tabular}
% \begin{tabular}{ccccccccccc}
% \toprule 
%  & KMNC & NBC & NC(0.0) & NC(0.2) & NC(0.5) & NC(0.75) & LSA & DSA & ANPC & SNPC\tabularnewline
% \hline\hline 
% % \midrule 
% SADL-1 & -0.262 & -0.262 & -0.300 & 0.099 & 0.315 & 0.001 & 0.000 & -0.638 & \textbf{\textbf{0.586}} & \textbf{0.723}\tabularnewline
% SADL-2 & -0.029 & -0.029 & \textbf{0.553} & -0.397 & -0.065 & -0.111 & 0.000 & 0.181 & \textbf{0.822} & \textbf{0.789}\tabularnewline
% VGG16 & -0.348 & -0.348 & 0.037 & -0.031 & -0.210 & -0.273 & 0.000 & -0.145 & 0.016 & -0.055\tabularnewline
% % \midrule
% \hline 
% Avg. & -0.213 & -0.213 & 0.096 & -0.109 & 0.013 & -0.128 & 0.000 & -0.201 & 0.475 & 0.486\tabularnewline
% % \bottomrule 
% \hline
% \end{tabular}
    \label{tab:corr}
\end{table*}



% or they are similar with other benign samples in the test suite. Meanwhile, we removed the same number of benign samples, which actually trigger more diverse decisions than the inserted adversarial samples. Thus, our coverage may decrease when more errors are introduced.

%The results show that natural errors could introduce more information (\ie, trigger different decision) than the adversarial examples.




\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ3:}} 
    Overall, ANPC and SNPC are more sensitive to different errors than other coverage criteria due to the CDP awareness. Different coverage criteria could achieve similar increasing trend, indicating that they tend to have some correlation.
    %Moreover, ANPC performs better in detecting adversarial examples while SNPC performs better in detecting natural errors. A promising direction might be to somehow combine them together (\ie, taking both control flow and data flow into consideration).
    
%The further analysis show that adversarial samples trigger limited decision logic than the natural errors.
%and the removed benign samples.
%By selecting suitable configuration (\ie, the number of the clusters and $\beta$), the path abstraction could further reduce the width of the path and achieve competitive results.
\end{tcolorbox}
\vspace{-.1in}
\subsection{RQ4: Correlation with Output Impartiality}
\revise{
As described in~\cite{ncmislead,test:deephunter,alshahwan2014coverage}, the test data or errors should be diverse in terms of the output.
The existing work~\cite{sekhon2019towards} has demonstrated that the coverage (\eg, neuron coverage) can be improved by a few samples. However, a test suite that only contains one category of samples (\eg, dog) is not enough to comprehensively reveal diverse defects of the DNN (\eg, the errors in other categories). In addition, the coverage criteria are usually used to guide the test case generation. The coverage criteria that are sensitive to output diversity can guide the testing tools to generate more diverse test cases belonging to different categories while the insensitive coverage criteria may generate biased test cases~\cite{test:deephunter}. Hence, we evaluate the correlation between the coverage criteria and the output diversity in this section.
}
\paragraph{Setup.} 
% The tests in a test suite should exercise more diverse output behavior with different decisions. The coverage criteria should be aware of the prediction bias~\cite{ncmislead}, \ie, the coverage should not be too high if most of the test cases have the similar prediction.
We follow the same setting in~\cite{ncmislead} and use the proposed tool to generate a number of test suites, which have the same size. 
\revise{Specifically, it mainly contains three steps:
\begin{enumerate}[leftmargin=*]
    \item For each dataset, we randomly select two seed test suites with different size (\ie, 100 and 500).
    \item Based on each seed test suite, we adopt the tool~\cite{ncmislead} to generate new test suites that have the same size with the seed test suite (\ie, generate new input by perturbing each input of the seed test suites). The tool~\cite{ncmislead} extends the existing adversarial attacks (\eg, C\&W ~\cite{cw2017} and PGD~\cite{madry2018towards}) with the divergence function such that more diverse test cases can be generated. By setting different configurations (\eg, diversity regularization weight, confidence), multiple test suites 
   can be generated. For each seed test suite on SADL-1, SADL-2, VGG-16 (CIFAR-10) and AlexNet, we generate 48, 171, 167 and 168 new test suites\footnote{The number of test suites is different because it depends on the number of configurations in~\cite{ncmislead} (\ie, a new test suite is generated by a configuration), where one variable in the configurations is the layers of the neuron network.}, respectively. 
   Note that, we did not include the results of ImageNet in this experiment because all adversarial examples generated by the tool~\cite{ncmislead} belong to the same class, which makes all correlation scores as NaN.
    \item For a generated test suite, we calculate the coverage and the output diversity, respectively. Finally, we calculate the \textit{Pearson vs Spearman} correlation between them.
\end{enumerate}
} 

% Specifically, we use the output impartiality metric~\cite{ncmislead} to represent the diversity of a test suite $X$:
% %Finally, for each configuration, we generate 48, 171, 167 and 168 test suites for SADL-1, SADL-2, VGG-16 and AlexNet, respectively. 
% For each test case, we calculate the coverage and the output diversity, then we calculate their correlation.
Specifically, we use the output impartiality metric~\cite{ncmislead} for a test suite $T$:
$$
output\_impartiality(T) = \frac{\sum_{t\in C_k}P_{t=C_k} logP_{t=C_k} }{\frac{1}{|c|}log\frac{1}{|c|}}
$$
where $|C|$ is the cardinality of classes and $P_{t=C_k}$ represents the
percentage of the test cases $t$ predicted to belong to class $C_k$. 

% \felix{missing figure and table refs below:}

%Figure~\ref{} visualizes the relationship between NPC/LNPC and the output impartiality and 
\paragraph{Results.} Table~\ref{tab:corr} shows the correlation on different models. The overall results demonstrated that, compared with existing coverage criteria, ANPC and SNPC are more strongly correlated with the output impartiality. In particular, we have the following findings:% 1) ANPC and SNPC have a weak correlation in VGG-16 when the size of the test suite is 100. Although some test suites are biased (\eg., there are many inputs predicted as 8 in one test suite), they still cover different CDPs (\ie, different decision logic), making the coverage high. 
1) Compared with the test suite with smaller size (\eg, 100),  the correlation can be stronger when the size of the test cases becomes larger (\ie, 500). For example, for the size 500, ANPC and SNPC are positively and strongly correlated with the output impartiality in all models while there are some negative correlation in the size 100. KMNC is also positively correlated with output impartially when the size is 500. 2) Consider the results of ANPC and SNPC, we found that SNPC is more strongly correlated with output comparability. It is because ANPC is more fine-grained and could capture the minor activation difference (\ie, coverage increase) even when they have output bias (\ie, the same prediction output). 


\revise{For the results that ANPC and SNPC achieve negative correlation (\eg, -0.244 on SADL-1, -0.055 on VGG16) when the size of the test suite is 100,  our in-depth analysis reveal that, for some test suites with smaller size,  the prediction outputs of the test cases are biased (\eg., these test cases are predicted as the same class), which caused the low output impartiality. However, these samples can still trigger different CDPs (\ie, different similarities compared with the corresponding CDP), which lead to high coverage. Hence, the correlation is negative. When the size becomes larger (\eg, 500), the test suite becomes more stable (\ie, the prediction results are less biased), which makes that the coverage is positively correlated with the output impartiality.
 }

\revise{We also observe that the correlation of IDC is higher than other baselines but it is still less than ANPC and SNPC. The average correlation scores of IDC are less than ANPC and SNPC. For example, when the size is 100, the average score of IDC is 0.298 while the average scores of ANPC and SNPC are 0.601 and 0.612, respectively. Except for VGG16 (size=100), all correlation scores of SNPC are larger than IDC. The results indicate the effectiveness of our fine-grained coverage criteria.}


% on SADL-1 and SADL-2. However, the correlation disappears in VGG16. Our in-depth analysis reveal that, NPC and LNPC measure how different the CDPs of test suites with recovered decision logic (\ie, different abstract CDPs) for the prediction of each class. Intuitively, the diverse CDPs in each class make NPC/LNC are more related to the output impartiality. It is interesting that the results of VGG16 have different results even it aims at the same task with SADL-2. We analyzed the similarity between the abstract CDP and CDPs of test cases in the test set, which has high coverage but output impartiality. We found that, although the prediction outputs of the inputs are biased (\eg., there are many inputs predicted as 8 in one test set), they still trigger more different CDPs which have different similarity with the corresponding CDP in the class 8. However, we execute the same test set in the SADL-2 and get relatively low coverage. The reason is that VGG16 is more complex than SADL-2, making it learn more diverse logic. As a result, some test cases are learned using the similar logic in SADL-2 but different decision logic in VGG16. 

% To further demonstrate it, we increase the size of the test set and found that the correlation increases. More detailed results are put int the website~\cite{deepnpc}. On the other hand, the existing coverage criteria do not take into account the output bias and have low correlation.



% . Thus, a test suite including more diverse outputs will trigger more diverse decision logic with regards to the corresponding class. However, the existing coverage criteria do
% not take into account the output bias and compare the neurons outputs universally, making them less sensitive with the output impartiality. The existing work has demonstrated that some specific class could achieve very high coverage (\eg, neuron coverage)~\cite{ncmislead,nerualmisled}.



\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ4:}}
Generally, ANPC and SNPC are positively correlated with the output impartiality.
The model and the size of test suite could affect the correlation.
%When the size of the test set is small, the correlation is not clear as the bias test cases could achieve high coverage. However, when the size of the test suite is large, improving the prediction diversity could further improve coverage.
\end{tcolorbox}
\vspace{-.1in}

\subsection{RQ5: Efficiency of NPC}
We use the same dataset from RQ3 and compare the time overhead of calculating the coverage of a test suite (\ie, 1000 samples). Note that, except for NC, all other coverage criteria depend on the training samples and there are some prepossessing process. For example, KMNC and NBC need to profile the training data. LSC and DSC need to calculate all activation values of the training data. ANPC and SNPC need to calculate the CDPs for all training data. IDC also requires the LRP calculation for all training data. Since the prepossessing phase can be executed only once and it is usually calculated offline, we ignore the time of the prepossessing and only compare the coverage calculation time for a given test set. 

Table~\ref{tab:time} shows the results. We found that, NC (with the threshold 0.0) is the most efficient one as it only depends on the neuron output. For ANPC and SNPC, we list the total time and the CDP path extraction time (the number in brackets).The results show that the path extraction is efficient. Compared with others, ANPC and SNPC take more time since more information are required (\ie, the CDP calculation). IDC is more efficient because it only calculates the distance between the 
critical neuron values of the test cases and the training samples at one layer.
Actually, it is a trade-off between effectiveness (\ie, leveraging more information) and the efficiency. 
%  DSC takes more time than ANPC and SNPC because it needs to compare the new input with all training samples. 

\begin{tcolorbox}[size=title]
	{\textbf{Answer to RQ5:}}
Although ANPC and SNPC adopt the interpretation analysis, the time overhead is not expensive. The CDP extraction is efficient and it only takes a proportion in the total time overhead of the coverage calculation. 
\end{tcolorbox}
\vspace{-.1in}


\begin{table}[!t]
    \centering
    \small
    \caption{The time overhead of coverage criteria on different models (seconds)}
    % Preview source code for paragraph 0

\begin{tabular}{ccccccccc}
\toprule 
 & ANPC & SNPC & KMNC & NBC & LSC & DSC & NC(0.0) & IDC\tabularnewline
\midrule 
\midrule
SADL-1 & 10.25(2.60) & 8.83(2.60) & 3.50 & 1.92 & 26.25 & 59.75 & 0.67 & 1.11\tabularnewline
SADL-2 & 39.50(14.45) & 47.33(14.45) & 26.75 & 13.67 & 24.67 & 166.17 & 1.33& 0.82\tabularnewline
VGG16(CIFAR-10) & 135.50(35.10) & 91.17(35.10) & 54.67 & 28.75 & 21.00 & 73.00 & 2.17& 2.81\tabularnewline
AlexNet & 57.00(13.35) & 29.50(13.35) & 104.33 & 53.25 & 37.08 & 136.00 & 1.08& 1.21\tabularnewline
\color{red}VGG16(ImageNet) & \color{red}203.24(59.67) & \color{red}119.75(59.67) & \color{red}146.43 & \color{red}88.02 & \color{red}154.27 & \color{red}173.27 & \color{red}30.45 &  \color{red} 13.21\tabularnewline
\bottomrule 
\end{tabular}

    \label{tab:time}
\end{table}

\section{Threats to Validity and Discussion}\label{sec:limit}
\paragraph{Threats to Validity}
\revise{
The internal threats to validity lies in our implementations including the LRP implementation, the path extraction, the path abstraction, the coverage criteria and the implementation in each experiment. To reduce this threat, the co-authors carefully checked the correctness of our implementation. 

The external threats to validity include the selection of the subjects and the tools used in the evaluation. Specifically, the selection of datasets and the used models could be a threat. To reduce this threat, we selected four widely-used subjects (MNIST, CIFAR-10, SVHN and ImageNet) and 4 DNNs (SADL-1, SADL-2, VGG-16 and AlexNet), where ImageNet is a large-scale dataset. Another threat could be the generated data including adversarial examples, the selected natural errors and test suites (in RQ3, RQ4 and RQ5). To mitigate this threat, we follow the same setting in the existing work~\cite{ncmislead,nerualmisled} and generate diverse data with multiple configurations. In addition, the usage of the existing tool~\cite{ncmislead} can be a threat. Since our method, the used models and the tool~\cite{ncmislead} are developed by PyTorch, we manually re-implement the tool~\cite{test:surprise,IDCcov} by PyTorch, which may not the exactly the same with the original version.  We integrate our method, LSC, DSC, NC, KMNC and NBC into the tool~\cite{ncmislead} to evaluate the correlation.
We carefully checked the code to mitigate the threat.

The construct threats mainly lie in the randomness, the selected baselines, the parameters. First, one threat is the randomness in the selection of the data. To mitigate the treat, in RQ3, we repeat each experiment 5 times (\eg, the generation of adversarial examples) and calculate the average results. In RQ4, we follow the setting~\cite{ncmislead} and generate a large number of test suites to reduce the randomness. Second, we adopted the state-of-the-art approaches that have been demonstrated to be insufficient in DL testing. We compare our method with them to demonstrate the advantages of our proposed coverage criteria. Thirdly, the hyper-parameters in our methods and the baselines could be a threat to validity.
To reduce the threat, for the baselines, we follow the settings in the existing works~\cite{ncmislead,test:surprise,ma2018deepgauge}. For our method, we set multiple configurations in terms of the hyper-parameters $\alpha$, $\beta$ and the number of clusters $k$. However, in RQ3 and RQ4, we select the same values of $\alpha$, $\beta$ and $k$ for all paths and classes. Actually, we can select the optimal configurations by adopting different $\alpha$, $\beta$ and $k$. In the future, we plan to evaluate our method with more configurations.
}

% First, the selection of subject datasets and DNNs could be a threat to validity. In this work, we try to select the widely-used datasets and models in the recent works. 
% Second, the configurable hyper-parameters could be a threat to validity such as $\alpha$, $\beta$, the number of clusters $k$ and the number of the buckets $m$. To counter this issue, we set different values of the parameters for comparison.
% In addition, the generated datasets (\eg, RQ3, RQ4, Rq5) may be a threat. To mitigate the threat, we randomly select multiple datasets and use the tool~\cite{ncmislead} with the same configuration to generate a large number of test suites for analysis. 

%widely used adversarial attack techniques to generate adversarial examples, and the tool~\cite{ncmislead} with the same configuration to generate a large number of test suites for correlation analysis. 


\paragraph{Limitation}
Like the coverage criteria in traditional software, we think there is no one best coverage criterion and each one has some limitations. The main advantage of NPC lies in its interpretability and the clear relationship with the internal decision of the DNN.
In this section, we summarize our limitation and discuss the potential solutions in the future.
\begin{itemize}
    \item Currently, our approach mainly considers the classification since the current interpretation technique (\ie, LRP) does not support the DNN with regression prediction. Even though the used interpretation technique is orthogonal with our approach, our approach is general as long as the critical neurons could be calculated.  We believe the interpretation techniques that work on regression tasks in the future will further solve this limitation.
    \item Our approach mainly works on feed-forward neural networks. For recurrent neural networks (RNNs), whose number of iterations is not fixed, it could be challenging for the interpretation technique (\eg, relevance calculation in LRP). In the future, we may extend LRP by unrolling the RNN to address this limitation.%This work only demonstrates that NPC is correlated with defect detection and output impartiality, and we did not evaluate the correlation with other properties, such as naturalness~\cite{ncmislead} and robustness enhancement~\cite{dong2019limited}. Actually, it is an open question about whether the testing criteria should be correlated with such properties. We leave the evaluation as the future work.
    \item \revise{There is another limitation on the selection for the number of the clusters during the path abstraction. Currently, we select the same number for all classes, which may not be the optimal setting. In the future, we will investigate the automated selection on this parameter.}
\end{itemize}


% 1) regression
% 2) how to cluster
% 3) evluation metrics: naturalness, robustness
% 4) RNN

==> sections-old/introduction.tex <==
\section{Introduction}
%
\begin{figure*}
    \centering
    % \includegraphics[width=0.8\linewidth]{pics/PathMov.pdf}
    \includegraphics[width=0.8\linewidth]{pics/PathMov_fx.pdf}
    \caption{(a) Difference between traditional software and DL software, (b) Paths in the DL software.}
    \label{fig:motivating}
\end{figure*}
%
Deep Learning (DL) have achieved tremendous success and demonstrated its great potential of solving complex tasks in many cutting-edge real-world applications such as image classification~\cite{app_img}, speech recognition~\cite{app_speech}, natural language processing~\cite{app_nlp} and software engineering tasks (\eg, commit message generation~\cite{commit_gen}, vulnerability detection~\cite{NIPS2019_9358} and clone detection~\cite{deckard}).
%
We have also seen an increasing demand to apply DL in some safety-critical areas, such as autonomous driving~\cite{ autodriving} and healthcare~\cite{medi_cancer}. However, Deep Neural Networks (DNNs) have been demonstrated with quality issues, \eg, to be vulnerable to adversarial attacks in spite of having achieved high accuracy~\cite{biggio2013evasion}. We have already witnessed the real-world cases caused by quality issues of DNNs, \eg, Tesla/Uber accidents~\cite{uber_crash} and incorrect diagnosis in healthcare~\cite{medi_cancer}. The systematic assessment of the quality of DNNs is urgently needed especially 
%before they are applied 
in safety- and security-critical scenarios.

Even until recently, the common way of quality evaluation of DNNs still mostly relies on train-validation-test splits to calculate the accuracy, which may over-estimate the performance of the model~\cite{ribeiro-etal-2020-beyond}. This motivates software engineering community to propose a variety of novel approaches and tools for systematically testing the quality of the DL software (\ie, the DNN). However, due to the fundamental difference between the traditional code-based software and the DL software (see Fig.~\ref{fig:motivating}(a)), the software testing techniques (\eg, code coverage) could not be directly applied in DL software, making testing of the DL software be a new challenge. 
%\qing{It is not clear for me about the reasons of `could not be directly applied'.}

To this end, inspired by the white-box testing of the traditional software, a number of approaches towards testing of DL systems have been recently proposed~\cite{nerualmisled}. Specifically, some structural coverage criteria are proposed to measure the test adequacy of the test suite via analyzing the internal neuron activities, \eg, Neuron Coverage (NC)~\cite{pei2017deepxplore}, its variants (\eg, KMNC, NBC, SNAC)~\cite{ma2018deepgauge}, the combinatorial testing based criteria~\cite{ma2019deepct,sekhon2019towards},
%which are built on the intuition of code coverage 
the Surprise Adequacy~\cite{test:surprise} and etc.
%which is based on the diversity of the test data. 
Based on the coverage criteria, automated testing techniques (\eg, DeepXplore~\cite{pei2017deepxplore}, DeepTest~\cite{tian2018deeptest} and DeepHunter~\cite{test:deephunter}) are further developed to generate test cases for maximizing the coverage. 

%The assumption is that the coverage criteria could measure the diversity of the model behaviors, and the testing tools aim to maximize the coverage such that more behaviors could be explored.

%The coverage criteria are assumed to measure the 
DNN testing aims to cover diverse internal decision logic of DNN such that more bugs (\ie, incorrect decisions) could be detected~\cite{sekhon2019towards,zhang2020machine}. 
Due to the black-box nature and complexity of DNNs, it is unknown and hard to understand the underlying principles of the existing coverage criteria~\cite{nerualmisled}. Specifically, for traditional software, the defects reside on particular instances of the program’s control and data flow~\cite{ma2019test}. Thus, the code-based coverage criteria (\eg, statement coverage, branch coverage) are meaningful and essential as covering more statements or branches is more likely to capture diverse behaviors (\ie, program logic) in terms of the control and data flow. However, unlike the traditional software, the decision logic of DNN is opaque to human, making it hard to understand the relationship between the decision logic and the existing coverage criteria. For example, it is not clear whether (de-)activating more neurons (\ie, NC) is better to capture more diverse behavior of the DNN. Thus one may wonder what is the semantics and meaning behind existing coverage criteria.  
%Although the proposed coverage criteria have shown some promising results~\cite{pei2017deepxplore,tian2018deeptest,test:deephunter}, it is still unknown about their the underlying principles due to the black-box nature and complexity of the DNN~\cite{ncmislead}. Specifically,
%code-based coverage criteria (\eg, statement coverage, branch coverage) are meaningful due to that the defects reside on particular instances of the program’s control and data flow~\cite{ma2019test}. It is intuitive that covering more statements or branches are more likely to capture diverse behaviors in terms of the control and data flow. 
%The test suite with high code coverage is more likely to capture more behaviors (\ie, the program logic) in terms of the control and data flow. 
%Similarly, the objective of DL testing is to test the internal decision logic such that more bugs (\ie, incorrect decision) could be detected~\cite{zhang2020machine,sekhon2019towards}. 
% However, one big challenge is that, unlike the traditional software, the decision logic of DNN is opaque to human, making it hard to understand the underlying principles of existing coverage criteria. For example, it is not clear whether activating more neurons (\ie, NC) is better to capture more behavior of the DNN. Thus one may wonder whether the existing coverage standards are meaningful. 
  
Some recent research~\cite{nerualmisled,dong2019limited,ncmislead,fsecorrelation} started to perform a more in-depth investigation of existing coverage criteria and have demonstrated their limitations in different perspectives. 
Harel-Canada et al. have shown that NC is neither positively nor strongly correlated with defect detection, naturalness and output impartiality ~\cite{ncmislead}. For example, their experimental results have shown that only a few inputs could already achieve 100\% NC~\cite{sekhon2019towards}. Li et al. demonstrated that the existing testing criteria are not effective or sensitive in distinguishing same-size test sets of \textit{natural} examples including different levels of misclassification rates~\cite{nerualmisled}. Dong et al. further showed that there is a limited correlation between the coverage criteria and the robustness of the DNN~\cite{dong2019limited}.  
These results force us to rethink what could be a better coverage criterion of DNN and how could we design more interpretable coverage criteria.
%In addition, Kim et al. claimed that the testing criteria should be able to guide the selection of inputs, which could be used to improve the accuracy of the DL system~\cite{test:surprise}. 


Motivated by the aforementioned challenges and limitations, in this paper, we propose coverage criteria from the new angle, called Neuron Path Coverage (NPC). We argue that a better coverage criterion should be more relevant to the decision logic of the DNN. To this end, NPC is designed to be \textit{interpretable}\footnote{\revise{We say that NPC is interpretable as it is designed to identify the key neurons that contribute more on the decision of the model based on the interpretation technique, \ie, Layer-Wise Relevance Propagation (LRP)~\cite{bach2015pixel}}} (\ie, easily understandable) and can better characterize the decision structure of the DNN.
In traditional software, a path in the control flow graph could represent the program logic of the software (\eg, the login, the logout, the invalid user input checking and etc.).
%which is \textit{interpretable} (\ie, easily understandable) and  \textit{effective} (\ie, better characterizing the decision structure of the DNN).
Inspired by this, we extract \textit{Critical Decision Paths} (CDPs) from the DNN, which represent the internal decision of the DNN on given inputs. For example, in Fig.~\ref{fig:motivating}(b), the DNN makes the decision along the corresponding CDPs (\eg, the yellow path or the red path), which is to classify the input as a dog or a cat. 
Based on the interpretation technique~\cite{bach2015pixel}, we extract \textit{critical} neurons in each layer, which dominate the decision of the DNN on the target input. The critical neurons between the layers form the CDP. Compared with the existing neuron-based coverage metric (\eg, NC~\cite{pei2017deepxplore}, $k$-multisection Neuron Coverage~\cite{ma2018deepgauge}, IDC~\cite{IDCcov}),
CDP considers not only the critical neurons in one layer but also the relationships among layers. Moreover, the CDP is clearly related to decision-making.
%Moreover, the CDP is more interpretable

%relationships between adjacent layers and the combinations of values of neurons in the same layer
%which are calculated from each of the intermediate layers. The CDP dominates the decision of the DNN on the target input, \eg, if they were suppressed to zeros, the final result would deteriorate severely.
%, the CDP is more interpretable, \ie, the relationship between the decision and the CDP is more easily understandable than the relationship between the decision and the activation of neurons.

%For example, it is hard to understand the relationship between  and it helps understand why the input is classified as the target class.

%first discuss and summarize the desired properties of the coverage criteria based on the existing works~\cite{dong2019limited,nerualmisled,ncmislead} (\cf, Section~\ref{sec:motivation}). Actually, it is a big challenge for one coverage criterion to satisfy all requirements and whether the coverage criteria should meet all of them is an open question. Our claim it that a better coverage criterion should meet the following properties: \ding{182} {it is interpretable, \ie, easily understandable}, \ding{183} {it is correlated with the defect detection~\cite{ncmislead,dong2019limited}}, \ding{184} {it is sensitive with the natural errors~\cite{dong2019limited,test:surprise}} and \ding{185} {it is correlated with the output impartiality~\cite{ncmislead}}. Furthermore, inspired by the path coverage in traditional software testing~\cite{pathcov}, we propose a new coverage criteria, called Neuron Path Coverage (NPC), for testing DL systems.  
We then recover the learned decision logic of the DNN by extracting CDPs from all training samples. Intuitively, the CDP can be regarded as the control flow of the DNN that shows the important decision logic. Hence, the objective of DL testing is to generate diverse test inputs that can trigger different decision logic (\ie, trigger different control/data flow of the DNN). We firstly construct a Decision Graph (DG) to represent the overall decision logics based on the training data. Since the number of training samples may be very large, we propose the path abstraction technique to build the abstract CDP. The abstract state represents the common decision logic that is shared by some inputs. 
%It is reasonable as the DNN is learned to be general such that the similar inputs could be handled with the similar decision logic (\ie, the CDP).
Based on the DG, we define two variants of path-based coverage criteria, named Structure-based Neuron Path Coverage (SNPC) and Activation-based Neuron Path Coverage (ANPC). Specifically, SNPC is designed based on the control-flow of the DNN (\ie, neurons in the path) while ANPC is designed based on the data-flow of the DNN (\ie, neuron activation values in the path).
An input can increase the coverage if it can trigger a different CDP or the similar CDP but with different activation values.


% Two variants of the path-based coverage criteria are proposed.
% Similar to paths in programs~\cite{pathcov}, the number of CDPs may be infinite in the DNN. To overcome such a challenge, we adopt a similar strategy~\cite{pathcov,test:surprise} by introducing parameters to bound the number of the paths, \ie, measuring the distance of the new CDP with the CDPs extracted from training samples. The number of training samples may be very large, which will introduce a high computational cost.
% %Specifically, we first extract CDPs from each of the training samples. 
% To improve the efficiency, we perform the path abstraction to calculate the abstract CDP, which is shared by the similar inputs (\ie, their decision logic is similar). The assumption is that the DNN has the generality to similar samples. Finally, we construct a Decision Graph (DG) based on the abstract CDPs. The DG is similar to the control flow graph of the program and represents the overall decision structure of the DNN.  We propose two variants of coverage criteria based on the control flow and data flow. The coverage criteria are measured by the distance between the CDP of new input and the CDPs in the DG. Intuitively, the larger the distance, the more diverse behaviors of the DNN are the more likely to be explored.


% Furthermore, we consider the concrete activation values of neurons in the CDP, which represents the data flow information of the corresponding CDP.
%The coverage criteria is expected to be correlated with the defect detection due to that the CDPs of the failed inputs (\eg, adversarial examples) are assumed to be different with the paths in the tree, which also explained why the DNN cannot handle it well.

To demonstrate the effectiveness of our techniques, we evaluate NPC on 4 widely-used datasets. Specifically, we first evaluate the accuracy of the extracted paths, \ie, whether they are critical and useful in explaining the decision of the DNN. Our results show that the CDPs are critical for the prediction of inputs. After masking the outputs along the CDPs, the prediction results are changed greatly (\eg, an average 98.9\% inconsistency rate). Moreover, the CDP is accurate to distinguish decision behaviors between different inputs in the same class. Then, we evaluate the usefulness of the proposed coverage criteria and the results show that NPC could distinguish the same-size test sets including a different number of natural errors. In addition, NPC is positively correlated with the output impartiality~\cite{ncmislead}, \ie, test set with high output bias has lower coverage. We also evaluate the efficiency of the coverage calculation, and the results show that the time overhead is not very expensive although NPC adopts the interpretation analysis. 
%However, after masking the outputs along the non-critical paths, the  predication is less affected (\eg, 1.2\% inconsistency rate).


In summary, this paper makes the following main contributions:
% \qing{Add the contribution for interpertable coverage criteria? }
\begin{itemize}
    %\item We analyzed the existing works and summarized the four desired properties for the coverage criteria.
\item We propose a method to construct a decision structure of the DNN based on the CDP extraction and abstraction.
\item Based on the decision structure, we propose two variants of coverage criteria that are more relevant to the decision-making logic of the DNN. 
%by measuring the internal decision effectively.%To the best of our knowledge, this is the first work to propose coverage criteria based on interpretation approach.
\item We conduct the comprehensive evaluation and demonstrate the effectiveness of the proposed approach. Our results show that the CDP is closely relevant to the decision-making; The proposed coverage criteria (\ie, SNPC and ANPC) are positively correlated with the detection of natural errors and output impartiality, respectively.%\ie, the interpretability of the CDP, the correlation between NPC and defect detection, 
\end{itemize}

%The remaining of this paper is organized as follows. Section~\ref{sec:motivation} introduces the background and our motivation. Section~\ref{sec:methodology} introduces our methodology including the construction of the decision structure and the neuron path coverage. Section~\ref{sec:eval} presents the evaluation results. Section~\ref{sec:realted} summarizes related work and Section~\ref{sec:con} concludes this work.


==> sections-old/motivation.tex <==
\section{Background and Motivation}\label{sec:motivation}
In this section, we briefly introduce software testing, the challenges of DL testing and the interpretation technique LRP.

\subsection{Traditional Software Testing}
Software testing has been widely studied in the past decades to evaluate the quality of the software. 
A central question of software testing is ``what is a test criterion?'', which defines what constitutes an adequate test~\cite{pathcov}.
In traditional software, the program logic is usually described by the programmer and can be represented as the control flow graph (see Fig.~\ref{fig:motivating}(a)). Based on the clear and easy-to-understand logic representation in the program, different coverage criteria have been proposed to measure the test adequacy, \eg, \textit{ statement coverage, branch coverage}, and \textit{path coverage}. These criteria are related to the program logic and the underlying principles are also intuitive: more program logic or behaviors could be explored by increasing the coverage (\eg, executing new statements or paths of the program).

\subsection{Challenges and Motivation}
Deep Neural Networks (DNNs) consist of multiple layers of neurons, which perform the nonlinear calculation for feature extraction and transformation. Similar to traditional software testing, the goal of DL testing is to test the decision logic of the DNN such that the incorrect prediction could be detected~\cite{sekhon2019towards}. However, unlike the control flow graph of the program, the logic of the DNN is opaque to humans, making it hard to design suitable coverage criteria. 
The neuron outputs of the DNN could reveal the behaviors of the DNN, thus some neuron outputs based coverage criteria~\cite{pei2017deepxplore,ma2018deepgauge,test:surprise} are proposed. However, it is not immediately clear how the neuron outputs reflect the internal decision logic, making it hard to understand its underlying principles and the meaningfulness of existing coverage criteria~\cite{nerualmisled}. 

The value range of neuron outputs is huge and it is often impractical to enumerate all possibilities. For efficiency, existing coverage criteria adopt different strategies to reduce the testing space. For example, NC~\cite{pei2017deepxplore} only considers two states (\ie, activated/inactivated) for the output of each neuron. $k$-multisection neuron coverage~\cite{ma2018deepgauge} discretizes the output value to $k$ buckets. Surprise metrics~\cite{test:surprise} select one of the layers to calculate the surprise score. The limitation is that it is unclear about the relationship between the coverage criteria and the decision logic of the DNN (\eg, whether a new decision-making behavior could be triggered by activating one neuron in NC). Consequently, if the coverage criteria are too coarse, some decision logic can be missed. For example, since NC is too coarse, several inputs can achieve very high neuron coverage~\cite{ncmislead,sekhon2019towards}. If the coverage criteria are too fine-grained, a huge number of inputs are needed. It is because many of them would trigger very similar decision logic with little difference.
The further results~\cite{sekhon2019towards,ncmislead,nerualmisled,dong2019limited} have also demonstrated the limitation of the existing coverage criteria, which call for new testing criteria design.

\noindent \fbox{
	\parbox{0.95\linewidth}{\textbf{Motivation}: Similar to the traditional software testing, a better coverage criterion for DL testing should be \textit{interpretable} and more closely \textit{related} to the decision logic of the DNN, which is what the existing coverage criteria lack. When new inputs increase the coverage, it is expected that new decision logic would be exercised and covered.
% 	This guide DL developers in an explicit way for testing.
%\qing{Add a sentence about existing criteria?}
	}
}
%which could better guide the test generation for detecting the defect detection. Motivated by this, in this paper, we aim to propose a new coverage criterion that is more directly relevant to the decision logic of the DNN. 

%For example, the coverage criteria are coarse~\cite{sekhon2019towards} and are neither positively nor strongly correlated to the defect detection~\cite{ncmislead,dong2019limited}.  

% For example, it is unclear whether activating a neuron  (NC) or a bucket ($k$-multisection neuron coverage) could trigger a new decision-making behavior

%Moreover, the coverage criteria are not effective if they are too coarse or fine-grained.  If the coverage criteria are too coarse, many useful inputs could be missed. For example, neuron coverage~\cite{pei2017deepxplore} is too coarse and the results have demonstrated that several inputs could achieve very high coverage~\cite{ncmislead,sekhon2019towards}. If the coverage criteria are too fine-grained (\eg, considering all possible neuron outputs), many redundant inputs could be generated, which reduces test efficiency.
%The further results~\cite{sekhon2019towards,ncmislead,nerualmisled,dong2019limited} have shown the limitation of the existing coverage criteria. For example, the coverage criteria are coarse~\cite{sekhon2019towards} and are neither positively nor strongly correlated to the defect detection~\cite{ncmislead,dong2019limited}.  




\subsection{Layer-Wise Relevance Propagation (LRP)}\label{sec:lrp}

\begin{figure*}
    \centering
    \includegraphics[width=.7\linewidth]{imgs/LRPExplain.pdf}
    \caption{\revise{Visualization of the LRP Process \cite{bach2015pixel}}}
    \label{fig:lrpvis}
\end{figure*}

\revise{
\begin{definition}
A Deep Neural Network (DNN) $f$
consists of multiple layers $\left\langle l_1,\ldots,l_n\right\rangle$, where $l_1$ is the input layer, $l_n$ is the output layer, and $l_2,\ldots,l_{n-1}$ are hidden layers. The inputs of each layer are from outputs of the previous layer.
\end{definition}

In this work, we mainly focus on the classifier $f:X \rightarrow Y $, where $X$ is a set of inputs and $Y$ is a set of classes.  Given an input $x\in X$, $f(x)=\argmax_{y}O_n$, where $O_n$ is a $|Y|$-dimensional vector, which is the output of the output layer $l_n$. The input is classified as the class $y$, and we use $g_f(x)=O_n(y)$ to represent the output value (\eg, the logits) for the class $y$.
%The output $y\in Y$ is the final prediction of the classifier.
Due to the complex non-linear calculation in the DNN, it is usually hard to understand the decision.




Layer-Wise Relevance Propagation (LRP)~\cite{bach2015pixel} is an effective way to interpret the decision by calculating the key features in the input. Given a $d$-dimensional input $x$ and the classifier $f$, $x$ is classified as the class $y$. To interpret the decision, LRP calculates the relevance (or contribution) of each dimension (\ie, pixel) in the input. Specifically, the classifier $f$ outputs $g_f(x)$ on the class $y$ and LRP calculates the relevance of each input dimension:
$$g_f(x) = \sum_{i=1}^{d} R_i^{l_1}$$
where $R_i^{l_1}$ represents the relevance of the dimension $i$ in the input layer $l_1$ (\eg, the pixel in an image). The sum of the relevance scores is equal to the output value $g_f(x)$, which means that each dimension can contribute to the final decision of predicting $y$ (\ie, $g_f(x)$). Intuitively, $ R_i^{l_1}<0$ contributes evidence against the presence of the class which is to be classified while $ R_i^{l_1}>0$ contributes evidence for its presence~\cite{bach2015pixel}. 


The relevance is calculated by a layer-by-layer backward propagation (from the output layer $l_n$ to the input layer $l_1$) such that:
$$g_f(x)=R_y^{l_n} = \sum_{i\in{l_{n-1}}} R_i^{l_{n-1}} = \ldots = \sum_{i\in{l_1}} R_i^{l_1}$$
where $R_i^{l}$ represents the relevance of the neuron $i$ at the layer $l$. The relevance calculation starts from the output neuron $y$ at the last layer $l_n$ (\ie, $R_y^{l_n}$) until the relevance $R_i^{l_1}$ of the input layer is calculated. At each layer, the sum of the relevance of all neurons is equal to the output $g_f(x)$. To be more specific, each relevance is calculated based on the following relation:  
$$R_j^{(l_{m+1})} = \sum_{i\in(l_m)} R_{i\leftarrow j}^{(l_m,l_{m+1})}, R_i^{(l_m)} = \sum_{j\in(l_{m+1})} R_{i\leftarrow j}^{(l_m,l_{m+1})}$$
where $R_j^{(l_{m+1})}$ represents the relevance of the neuron $j$ at the layer $l_{m+1}$, $R_{i\leftarrow j}^{(l_m,l_{m+1})}$ represents the relevance of the neuron $i$ at the layer $l_m$, where the output of the neuron $i$ is the input of the neuron $j$ at the layer $l_{m+1}$.
The relevance calculation starts from the output neuron at the last layer $l_n$ is $R_y^{(l_n)}=g_f(x)$ until the relevance $R_i^{(1)}$ of the first layer (\ie, the input layer) is calculated. 

Fig.~\ref{fig:lrpvis} shows the LRP calculation process on an image. In the left box, we show the ``black-box'' prediction where the image is classified as a dog and outputs $g_f(x)$. 
To interpret why it is classified as the dog, LRP calculates the relevance layer-by-layer starting from the output $g_f(x)$ (shown in the right box). Finally, neurons/pixels that have more impact on the prediction are identified. 


%Please refer to~\cite{bach2015pixel} for more details about the backward relevance calculation.

}

==> sections-old/relatedwork.tex <==
\section{Related Work}\label{sec:realted}
This section summarizes the related work on DL testing and adversarial attacks.
\subsection{DL Testing}
DeepXplore \cite{pei2017deepxplore} proposes the first white-box coverage criteria, \ie, Neuron Coverage, which calculates the percentage of activated neurons. A differential testing approach is proposed to detect the errors by increasing NC. DeepGauge \cite{ma2018deepgauge} then extends NC and proposes a set of more fine-grained coverage criteria by considering the distribution of the neuron outputs from training data. 


Inspired by the coverage criteria in traditional software testing, some coverage metrics~\cite{sun2018concolic,ma2019deepct,ma2018deepmutation} are proposed. DeepCover \cite{sun2018concolic} proposes the MC/DC coverage of DNNs based on the dependence between neurons in adjacent layers. 
 DeepCT~\cite{ma2019deepct} adopts the combinatorial testing idea and proposes a coverage metric that considers the combination of different neurons at each layer. 
DeepMutation \cite{ma2018deepmutation} adopts the mutation testing into DL testing and proposes a set of operators to generate mutants of the DNN.
%modified code/decision coverage in software testing, 
Furthermore, Sekhon \etal \cite{sekhon2019towards} analyze the limitation of exiting coverage criteria and propose a more fine-grained coverage metric that considers both of the relationships between two adjacent layers and the combinations of values of neurons at each layer. 

Based on the neuron coverage, DeepPath~\cite{wang2019deeppath} initially proposes the path-driven coverage criteria, which considers the sequentially linked connections of the DNN. Although both of DeepPath and our method focus on path-based coverage, the approach and the underlying principles are totally different. The path in DeepPath is the \textit{syntactic} connections between neurons in different layers and the semantics of the path is unknown. Differently, we adopt the interpretation techniques to define paths, in which the neurons are selected based on the relevance with the decision. Thus, CDPs have more clear \textit{semantics}, \ie, they are related to the decision logic. 

The aforementioned techniques mainly consider syntactic structure of DNN, which is black-box and hard to understand. Differently, Kim \etal \cite{test:surprise} proposed the coverage criteria that measure the surprise of the inputs. The assumption is that surprising inputs introduce more diverse data such that more behaviors could be tested. Surprise metric measures the surprise score by considering \textit{all} neuron outputs of one or several layers. It is still unclear how the surprise coverage (calculated from some layers) is related to the decision logic. Differently, our method not only selects the \textit{critical} neurons at each layer but also considers the relationships between layers.

Based on the these criteria, some automated testing techniques \cite{pei2017deepxplore,tian2018deeptest,test:deephunter,odena2018tensorfuzz,sun2018concolic} are proposed to generate test inputs towards increasing the coverage.
In addition, while the coverage criteria are widely studied, the existing work~\cite{dong2019limited,ncmislead,nerualmisled,sekhon2019towards,fsecorrelation,DeepGini} found some preliminary evidence about the limitation of the \textit{structural} criteria. For example, the coverage is too coarse and is not correlated to the defect detection and robustness. Such findings motivate this work that proposes \textit{interpretable} coverage criteria by extracting the semantic structure (\ie, the decision graph).

Recently, some coverage criteria~\cite{decisiontreeCov,IDCcov} are also proposed based on the decision of the DNN. The technique~\cite{decisiontreeCov} adopts the explanation technique LIME~\cite{lime} to extract a decision tree that explains the decision of the DNN on an input. Based on the decision tree, the symbolic execution is used to generate test cases that can maximize the path coverage on the decision tree. Different with~\cite{decisiontreeCov}, we extract the decision graph that could represent the global decision behaviors of the DNN. Moreover, in~\cite{decisiontreeCov}, it mainly focuses on problem of fairness evaluation while it is hard to extract such a decision tree on the high dimensional data such as image domain. IDC~\cite{IDCcov} adopts the interpretation technique to select the important neurons in one layer. Based on the training data, it then groups the activation values of important neurons into a set of clusters and uses the clusters to measure the coverage. Similar with our technique, IDC also selects the critical neurons. Differently, NPC considers the relations between layers and proposes the path-based coverage instead of only one layer. Thus, NPC does not need to select one of the target layer. In addition, we propose two different path coverage criteria from the control flow and data flow of the DNN.
For more relevant discussion on the recent progress of machine learning testing, we refer the interesting readers to the recent comprehensive survey~\cite{zhang2020machine}.

\subsection{Adversarial Attacks}
Recently, there are many adversarial attack techniques such as \emph{FGSM}~\cite{Goodfellow2015}, \emph{JSMA}~\cite{papernot2016SP}, \emph{BIM}~\cite{Kurakin2017adver}, \emph{DeepFool}~\cite{Seyed2016DeepFool} and \emph{C\&W}~\cite{cw2017}.
% \lei{cite PGD attack}
The adversarial examples are generated by adding visually imperceptible, perturbation to an input such that the new input is misclassified. It is worth to think and discuss about the difference between deep learning testing and adversarial attacks. The common thing is that both of the testing and attack could test the robustness of the model by generating incorrect inputs. Differently, the adversarial attack is ad-hoc and generates the \textit{specific} adversarial examples based on gradient calculation. 
DL testing aims to test the DNN more systematically by exploring more decision logic of the model. Thus, the errors generated by DL testing are expected to be more diverse (\ie, triggering different logic) than adversarial attacks. For example, given one input, the attack techniques usually generate the similar adversarial examples while DL testing could generate different adversarial examples with the guidance of the coverage criteria.



\section{Conclusion}\label{sec:con}
Motivated by the recent findings \cite{ncmislead,nerualmisled,dong2019limited} about the limitation of the existing DL testing criteria, this paper proposes the neuron path coverage via extracting the decision structure of the targeted DNN. For a DNN, we extract the decision logic based on the critical decision paths from the training data. Two path-based coverage criteria are then proposed. To the best of our knowledge, this is the first work that proposes the interpretable coverage criteria from the control-flow and data-flow of the DNN. The evaluation results demonstrated the effectiveness of the CDP in the decision revealing of the DNN and the usefulness of the coverage criteria.

%Compared with the existing structural coverage criteria, the proposed path coverage criteria are interpretable.
